Neighbor Auto-Grouping Graph Neural Networks for Handover Parameter Configuration in Cellular Network

The mobile communication enabled by cellular networks is the one of the main foundations of our modern society. Optimizing the performance of cellular networks and providing massive connectivity with improved coverage and user experience has a considerable social and economic impact on our daily life. This performance relies heavily on the configuration of the network parameters. However, with the massive increase in both the size and complexity of cellular networks, network management, especially parameter configuration, is becoming complicated. The current practice, which relies largely on experts' prior knowledge, is not adequate and will require lots of domain experts and high maintenance costs. In this work, we propose a learning-based framework for handover parameter configuration. The key challenge, in this case, is to tackle the complicated dependencies between neighboring cells and jointly optimize the whole network. Our framework addresses this challenge in two ways. First, we introduce a novel approach to imitate how the network responds to different network states and parameter values, called auto-grouping graph convolutional network (AG-GCN). During the parameter configuration stage, instead of solving the global optimization problem, we design a local multi-objective optimization strategy where each cell considers several local performance metrics to balance its own performance and its neighbors. We evaluate our proposed algorithm via a simulator constructed using real network data. We demonstrate that the handover parameters our model can find, achieve better average network throughput compared to those recommended by experts as well as alternative baselines, which can bring better network quality and stability. It has the potential to massively reduce costs arising from human expert intervention and maintenance.

==> sections/ActionOpt.tex <==
In this section we present our algorithm for action configuration where based on our trained reward model, one action per day is recommended for each cell.
The goal is to find the best action for cell $v$ at day $t$, i.e. $a_t^{v}\in{\mathcal A}$, that optimizes the problem in (\ref{eq:opt}).

As discussed in the earlier sections the main objectives to consider in the action configuration process are load balancing, identified by the throughput ratio, and the cell throughput. In general, when dealing with a multi-objective problem, different objectives are often conflicting, and we may not be able to optimize them simultaneously. {{One common way to tackle this problem is to give different objectives weights and optimize the weighted objective value. However, in our scenario, it is difficult to determine the weights and different clusters may require cluster-specific weights.}} Here we break the problem in (\ref{eq:opt}) into two sub-problems, and solve them sequentially. We first optimize the action with respect to the predicted throughput ratio, i.e., $\hat{\beta}_{t+1}^{v}(a_t^{v})$ for cell $v$ at day $t$, where $a_t^{v}\in{\mathcal A}$, and then optimize the throughput $\hat{\alpha}_{t+1}^{v}(a_t^{v})$.

Specifically, the throughput ratio is optimized and we find the set of best $c$ values for $a_t^{v}$, denoted $\mathcal A_c^{v}$, such that 
\begin{equation}
    \min_{a_t^{v}\in{\mathcal A_c^{v}}}-\sqrt{\big|1-\hat{\beta}_{t+1}^{v}(a_t^{v})\big|}\ge\max_{a_t^{v}\in{\mathcal A}-{\mathcal A_c^{v}}}-\sqrt{\big|1-\hat{\beta}_{t+1}^{v}(a_t^{v})\big|}.
\end{equation}
Then, our goal is to achieve the maximum possible throughput for cell $v$ at day $t$ and this is through
\vspace{-0.1cm}
\begin{equation}
    \hat{a}_t^v = \argmax_{a_t^{v}\in\mathcal A_c^{v}}~\hat{\alpha}_{t+1}^{v}(a_t^{v}).
\end{equation}
\vspace{-0.1cm}
% Finally the selected action are converted into the original range of $[-A,+A]$ to find the A2-threshold-RSRP parameter for the next day.
$\hat{a}_t^v$ is then the final recommended action for cell $v$ at day $t$. This procedure for all the $N_t$ cells of the network at day $t$ is presented in Fig.\ref{fig:optimizer} and Alg.~\ref{alg}.

\begin{figure}[t!]
	\centering
	\vspace{-.2cm}
	\includegraphics[width=.35\textwidth]{figures/optimizer.pdf}
	\vspace{-.6cm}
	\caption{Schematic of the multi-objective optimizer used for action recommendation based on the two trained models.}
	\vspace{-.4cm}
	\label{fig:optimizer}
\end{figure}

%\setlength{\textfloatsep}{0pt}

\begin{figure}
\vspace{-.2cm}
\begin{algorithm}[H]
\caption{TAG-GCN for Action Configuration}
\label{alg}
\textbf{Input}: $\textbf{P}_t^v$ and $\textbf{x}_t^u$ where, $u\in\mathcal{N}_t(v)$ $\forall j\in[1,N_t]$ \\
% \textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: $a_t^{v}$ for $\forall v\in[1,N_t]$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $v = 1$ and $\forall j\in[1,N_t]$ set $\mathcal A_c^{j}=\emptyset$.
\WHILE{$v\le N_t$}
\STATE Feed the TAG-GCN model with $\textbf{P}_t^v$ and $\textbf{x}_t^u$, for all neighbor $u\in\mathcal{N}_t(v)$.
\STATE Freeze all inputs of TAG-GCN except actions and predict the performance metrics $\hat{\alpha}_{t+1}^{v}(\cdot)$ and $\hat{\beta}_{t+1}^{v}(\cdot)$ for the input actions.
\FOR{$|\mathcal A_c^{v}|\le l$}
\STATE $x = \argmax_{a\in\{\mathcal A-\mathcal A_c^{v}\}}-\sqrt{\big|1-\hat{\beta}_{t+1}^{v}(a)\big|}$\;
  \STATE $\mathcal A_c^{v} = \mathcal A_c^{v} \cup \{x\}$
\ENDFOR
\STATE $a_t^{v} = \argmax_{a\in\mathcal A_c^{v}}\hat{\alpha}_{t+1}^{v}(a)$ \;
\STATE $v = v+1$
\ENDWHILE
\STATE \textbf{return} $a_t^{v}$ for $\forall v\in[1,N_t]$
\end{algorithmic}
\end{algorithm}
\vspace{-.9cm}
\end{figure}

==> sections/Introduction.tex <==
The rapid growth in the demand for mobile communication for new emerging technologies such as the Internet of Things (IoT), autonomous driving, and robotics makes it essential to improve cellular network performance. A cellular network is formed by many cells distributed over land areas, each served by at least one fixed-location base station (BS). 
These BSs provide wireless links with network coverage. A wide geographic area coverage can be achieved by having multiple cells to support many users. 
%Cellular networks provide advanced features such as increased capacity by saving frequency bandwidth, low power consumption, and larger coverage by adding cells with no limit over alternative solutions \cite{miao2016fundamentals, tekinay1991handover}.

% One of the factors that have a significant impact on the quality of service (QoS) in such networks is the handover function \cite{tekinay1991handover}.
% The cell BS is responsible for monitoring the level of the received signals by served users, which can be degraded when a user travels from one cell to another, and trigger a handover process in the proper moment to transfer the user to another cell BS that is receiving the strongest signals without interrupting the user data transmission.

The performance of a cellular network relies heavily on its parameter configurations. These parameters govern access control, handover, and resource management \cite{dahlman20134g, cellularOpt}. 
As the number of mobile users continues to grow rapidly, optimizing the parameter configurations of cellular network is becoming crucial \cite{mobile_users}. One of the factors that has a significant impact on the quality of service (QoS) in such networks is the handover parameter~\cite{tekinay1991handover}.
The cell BS is responsible for monitoring the strength of the signals received by served users, which can degrade when a user travels from one cell to another. The BS should trigger a handover process at the proper moment to transfer the user to another cell BS that is receiving the strongest signals. It is important not to interrupt the user data transmission. Thus, appropriately setting the parameter configuration that controls the handover process between cells is vital.
Due to the dynamic nature of the environment, any employed algorithm for parameter configuration should be capable of tracking the non-stationary changes in the environment, i.e., fluctuations of user number, network load, etc., and configuring the parameters suitably over time \cite{agiwal2016next}. 
Also, due to the diverse characteristics of cells across the network, the best parameter configuration for one cell may not be optimal for another \cite{dahlman20134g}. 
Consequently, developing an algorithm that can adapt to the temporal dynamics and cell diversity in real networks is essential for parameter configuration \cite{jiang2016machine}.

The current cellular network deployments are highly dependent on human experience. An expert designs rules or analytical models based on domain knowledge and assumptions about the network dynamics.
This approach is far from optimal. First, the human-designed rules/models only consider a limited number of network states (e.g., user distribution, channel quality, etc.) and parameters, and cannot capture the complex relationships between network states, parameter configurations and network performance.
Second, the assumptions of the network dynamics, based on which the rules/models are developed, are often simplified without considering the non-stationary changes in real environments, which degrades their performance. Finally, these rules/models may not be able to deal with the cell diversities in the network which makes them sub-optimal \cite{challengesOpt}.

Recently, data-driven approaches based on machine learning (ML) have been extensively used for parameter configuration and network management in cellular networks \cite{yuliu2017, hamilton2017, tabfar2012, riihijarvi2018machine, infocom_dlCell, dynamicprogramming}.
It has been shown that the multi-layer perceptron (MLP) can be considered as a universal function approximator \cite{goodfellow2016deep}.
Thus, in environments such as cellular networks where there is lack of an accurate analytical model and the network is highly dynamic, neural-network-based methods can be used to achieve high accuracy prediction.
ML models can utilize high dimensional information and approximate complex functions to fully describe the relationship between network states, parameter configurations and network performance metrics, which cannot be achieved by human experience. 

One of the key challenges in the network parameter optimization problem is the complex spatial and temporal dependencies in the cellular network. The parameter configuration of one cell not only affects its own performance, but also affects its neighbors'. Therefore, there are strong interactions between neighboring cells. When the network is heterogeneous, these interactions become extremely complex. Furthermore, the network states are often temporally correlated. Therefore, we would like to investigate two important questions: {1) \textit{\textbf{Modeling}}: how to model the spatial and temporal dependencies of the cellular network? 2) \textit{\textbf{Decision-making}}: how to choose the parameter values to jointly optimize the overall performance of interconnected and interacting cells?}


In this work, first we propose a model to precisely imitate the cellular network environment and then, we use this model to configure the parameters.
In order to address the above challenges, for each center cell surrounded by some neighbors, we define a novel method to consider the adjacent cells and differentiate their impact on the center cell.
This model helps capture the spatial interactions and the network heterogeneity.
We also consider the changing dynamics of the network to capture the temporal dependencies.
 Finally, to optimize the global network throughput, we introduce a local multi-objective optimization strategy to balance the center cell's load with its neighbors'  while increasing their throughput.
Our main contributions are summarized as follows. We:
\begin{itemize}
    \item Propose a novel method to model the impact from the neighbors of each cell in a distinguishable way to capture the complex spatial dependencies of the network.
    \item Consider  the changing dynamics of the network in our reward model to better reflect the temporal dependencies of the network.
    \item Introduce a multi-objective optimization strategy based on the model to consider several performance metrics and improve the overall network throughput.
\end{itemize}

In this paper, we consider the case of handover parameter optimization in cellular networks since it is one of the most common scenarios where strong interactions exist between neighboring cells. 
High speed user equipments (UEs) such as autonomous vehicles need effective and efficient handover procedures to guarantee minimum service delay or interruption. Also the increase in the number of service stations (due to the increasing number of UEs) causes frequent service area changes for UEs, and this must be handled effectively. 

The adjustment of handover parameters can dramatically affect the network throughput in several ways \cite{ltestd}. First it helps balance the traffic load in the network. Consider the A2-threshold parameter as an example. During the handover process in cellular networks, in order to guarantee an acceptable service quality, a UE must monitor the Reference Signal Received Power (RSRP) of the serving cell \cite{ltestd}.
As soon as the RSRP drops below the pre-defined A2-threshold, the UE starts to report measurements to its serving cell and prepares for handover. 
When this threshold is set higher, more UEs in the serving cell are triggered for handover, and this spreads the serving cell's load to its neighbors, resulting in a significant change of throughput for the serving cell and its neighbors.

Apart from the effect of load balancing, the handover parameters also impact a cell's throughput via other mechanisms. For example, small values of the A2-threshold cause a very poor experience for edge UEs and lead to repeated connection loss. On the other hand, the handover process is too frequent if the threshold is too large. This requires a considerable amount of bandwidth for measurement reporting and causes a drop in data throughput.

Due to the reasons outlined above, when optimizing this parameter, cell interactions must be considered and an accurate optimization process is of high importance for the network overall performance. This requires an accurate model to mimic network behavior and an optimization strategy to achieve the highest possible network throughput.

The rest of this paper is organized as follows. 
We first present some of the existing works on handover optimization and the load balancing problem in Sec.~\ref{sec:related_work}.
In Sec.~\ref{sec:problemFormulate}, we formulate the parameter optimization problem in cellular networks.
% We present the graph structure for data aggregation in Section \ref{sec:graphData}.
Our model is proposed in Sec.~\ref{sec:mlpmodel}.
We present our parameter configuration strategy in Sec.~\ref{sec:opt}.
In Sec.~\ref{sec:simulation}, the simulation results are demonstrated, and some concluding remarks are presented in Sec.~\ref{sec:conclu}.
More details are also provided in Appendix~\ref{sec:app}.

==> sections/ProblemForm.tex <==
In this section, we introduce the optimization problem for handover parameter configuration. Consider a network with $N$ cells, and form $N$ clusters each composed of one of the network cells as its center cell along with its neighboring cells. We elaborate the definition of neighboring cells in Sec.~\ref{sec:mlpmodel}.
The parameter we are optimizing is the one mentioned in Sec.~\ref{sec:introduction}, namely the A2-threshold, and we choose it as an example to investigate the performance of our algorithm. According to the 3GPP standard \cite{ltestd}, an A2 event is triggered when the received power at user $u$ from cell $n$, $P^{u,n}$, satisfies
\begin{equation}\label{eq:A2_event}
    P^{u,n} + H_{ys} < Thresh,
\end{equation}
where $H_{ys}$ is the hysteresis parameter to avoid frequent handovers and $Thresh$ is the A2-threshold we are optimizing.
Fig.~\ref{fig:cells} shows a cluster in a cellular network where user $u$ is crossing one cell's coverage area and monitors the received power from cell $n$ to check the handover criteria. 

\begin{figure}[t]
    \vspace{-.1cm}
    \centering
    \includegraphics[width=.35\textwidth]{figures/cells.pdf}
    \vspace{-.55cm}
    \caption{A typical structure of a cluster in the cellular network serving different types of users.}
    \vspace{-.6cm}
    \label{fig:cells}
\end{figure}

We consider an online optimization process. In real practice, network operators are often conservative and only allow a limited number of experiments. Let us assume that the optimization period has $L$ days, and the A2-threshold can be adjusted once for each cell at the beginning of each day. For day $t$, let $D_t$ be the total bits transmitted by all the cells, and $T_t$ be the total transmission time. We would like to maximize the accumulated network throughput of the optimization period, i.e.,
\vspace{-0.2cm}
\begin{equation}\label{eq:throughput}
    \max \sum_{t=1}^L \frac{D_t}{T_t}.
\end{equation}
\vspace{-0.2cm}

Maximizing the overall network throughput by jointly optimizing the A2-threshold of all cells is difficult. The problem becomes even more complicated as the network size increases, which makes a centralized solution not scalable. The adjustment of the A2-threshold of one cell only affects its local neighborhood. In this paper, we convert the centralized problem into a local decision problem. That is, each cell only examines its local performance metrics and chooses its own parameter configuration value.

As discussed in Sec.~\ref{sec:introduction}, the adjustment of the A2-threshold affects the network throughput via two means: better resource utilization by load balancing, and improved cell throughput with less connection loss and measurement reporting. Consequently, in order to configure the A2-threshold, these two metrics must be considered in the local decision problem. 

The throughput of cell $i$ at day $t$ is highly dependent on its A2-threshold $a_t^i$, denoted as $\alpha_t^{i}(a_t^i)$. The load balancing factor in the $i$-th cluster with center cell $i$ at day $t$ with A2-threshold $a_t^i$ is defined as the ratio of the center cell throughput to the average throughput of its neighboring cells, denoted by $\beta_t^{i}(a_t^i)$ and formulated as follows:
% \vspace{-0.1cm}
\begin{equation}
    \beta_t^{i}(a_t^i) = \frac{\alpha_t^{i}(a_t^i)}{\bar{\alpha}_t^{i}(a_t^i)},
\end{equation}
% \vspace{-0.1cm}
where $\bar{\alpha}_t^{i}(a_t^i)$ is the average throughput of the neighbors of cell $i$ with action $a_t^i$ and, denoting by $\mathcal{N}_t(i)$ the set of all neighbors of cell $i$ at day $t$, it can be formulated as:
\begin{equation}
    \bar{\alpha}_t^{i}(a_t^i) = \frac{1}{\vert \mathcal{N}_t(i) \vert}\sum_{j \in \mathcal{N}_t(i)}\alpha_t^{j}(a_t^i).
\end{equation}
The throughput ratio (rather than traffic/user ratio) is used since different cells have different capacities. This value approaches $1$ when loads of different cells match their capacities.

Our goal is to maximize the overall network throughput by optimizing the two important network performance metrics, namely, throughput ratio $\beta_t^{i}(a_t^i)$ and throughput $\alpha_t^{i}(a_t^i)$ for each cell $i\in[1,N_t]$, where $N_t$ is the total number of cells at day $t$, at the same time.
Therefore, we propose the following optimization problem for tuning the A2-threshold for cell $i$:
% \begin{align}\label{eq:opt}\nonumber
%     \argmax_{a\in\mathcal A}&~~-\sqrt{\big|1-\beta_t^{i}(a)\big|},\\
%     \argmax_{a\in\mathcal A}&~~\alpha_t^{i}(a),
% \end{align}
\vspace{-0.1cm}
\begin{equation}\label{eq:opt}
    \argmax_{a_t^i\in\mathcal A}\Big(-\sqrt{\big|1-\beta_t^{i}(a_t^i)\big|}, \alpha_t^{i}(a_t^i)\Big),
\end{equation}
\vspace{-0.1cm}
where $\mathcal A$ is the set of all possible values for the A2-threshold in the cellular network.

The challenge of solving the above problem lies in several folds. \textit{First}, since the network performance function is complex, dynamic and unknown, obtaining accurate $\beta_t^{i}(a_t^i)$  and $\alpha_t^{i}(a_t^i)$ is difficult. Instead, in this work, we adopt a data-driven approach where we learn reward models to estimate the performance metrics. \textit{Second}, in real-world cases, only a limited experimental budget is allowed by network operators. There will not be enough diverse historical data (state, action pairs) to train a data-driven learning model. In our design, we use a data augmentation technique in the form of neighbor cell augmentation to enrich the features from each cell. \textit{Third}, the handover parameter configuration is affected by adjacent cells. Thus, it is essential to model the information coming from the adjacent cells to achieve accurate reward modeling. In Sec.~\ref{sec:mlpmodel}, we present a novel method to accurately model the information from the neighboring cells that better suits the cellular network modeling. \textit{Lastly}, optimizing one performance metric greedily might hinder another performance metric, thus, how to jointly optimize different performance metrics needs careful consideration. In Sec.~\ref{sec:opt}, we propose a simple and effective solution to choose the desired handover parameters (actions) by considering multiple objectives. We will elaborate upon our design, which addresses these challenges, in the following sections.


==> sections/RelatedWork.tex <==
% \subsection{Common Handover Measures and Parameters}
% As it has been stated, the increase in the number of UEs which mostly require high bandwidth and heavily rely on short or non-existing service delays or interruptions escalates the urgency of optimal wireless network configuration. Among the crucial parameters in the network that play a vital role in providing such services are the parameters corresponding to handover (HO) events. High speed UEs such as autonomous vehicles need effective and efficient handover procedures to guarantee minimum service delay or interruption. Also the increase in the number of service stations (due to increase of the number of UEs) causes frequent service area crossing in the UEs which, again, requires proper handling techniques. 

Due to its importance, handover parameter optimization has been  the focus of a considerable research effort. To assess the effectiveness of their proposed algorithms for optimizing handover parameters, researchers use different measures such as handover failure (HOF) rate, handover frequency, Ping-Pong (PP) rate, network throughput, and load balancing.  When performing optimization in a real network, some of these measures may conflict. 
Therefore, it is crucial to consider a combination of these quantities to find a solution that satisfies different requirements of the network.

There are multiple parameters that impact handover in a network. These parameters generally are grouped in three categories. {\em RSRP and RSRQ} parameters are indicators of the signal strength and quality of the serving station, respectively, {\em Hysteresis} parameters act as a tolerance margin to avoid the PP effect, and {\em Time To Trigger (TTT)} parameters  are set such that short term violations of handover conditions are ignored to avoid the PP effect. We now review some of the existing works on handover parameter optimization.

\subsection{Traditional Handover Optimization Methods}

A wide variety of methods have been used for managing handovers in a wireless network. Fuzzy system handover algorithms, for example, have been used in several techniques. In \cite{vasmah2012}, Vasu et al.\ design an effective set of fuzzy rules based on different measures of the quality-of-service (QoS) in the network. Such techniques are accurate and stable due to deterministic rules, however designing proper rules for such a complex problem is not an easy task. Moreover, the set of rules for optimal functioning of the network will become increasingly complex and therefore not manageable.

\subsection{Machine Learning and Reinforcement Learning Methods}
Data-driven based approaches have beeb drawing increasing attention in the past decade. Advanced ML techniques (e.g., Reinforcement Learning (RL)) have been used in mobility management and handover optimization. These models are an efficient tool for the task of handover optimization because they can model non-linear functions and adapt to highly dynamic environments. Many studies show that the use of RL methods with fuzzy systems can improve performance~\cite{wuliu2015, klekur2013, munbar2013, dinkuk2013}. In \cite{wuliu2015}, Wu et al.\ try to properly adjust the handover margin to improve call drop ratio (CDR). The method in \cite{klekur2013}, uses the HOF rate as its measure for improvement and the input parameters are TTT and Hysteresis. Although measures of HOF rate and CDR are important in terms of user experience, the actual throughput that is delivered to the users is also a very important measure. This issue is tackled partially in \cite{munbar2013}, which describes a method that adjusts the transmission power (TXP) and the Hysteresis in small BSs to improve the balance of the load in the network. Load balancing is also considered in \cite{dinkuk2013} as an optimization objective; the developed technique adjusts the Hysteresis and TTT parameters simultaneously, while a heuristic algorithm optimizes the handover offset according to load measurements in the cell. 
% Also in \cite{munbar2015}, the authors introduce an algorithm that considers load balancing and handover optimization jointly as measures. 
% They first use a Fuzzy System (FS) to generate the action. This FS uses CBR (Call Blocking Ratio), HOR (Handover Rate), and HOM (Handover Margin) to produce an optimum HOM. Standard FS have one output. However, the authors in this paper design a FS with two outputs and the inference engine contains rules with two possible outputs. To choose the best action in these cases, they have used a Q-Learning scheme. It is important to note that in the aforementioned methods, throughput is never considered as an optimization objective. Moreover, only limited information (parameter values) from immediate neighbors is used to achieve the objectives while load balancing can be done more effectively when there is more information available from the neighboring stations.

Deep reinforcement learning (DRL) is another technique that has been used to solve the handover optimization problem. In \cite{caolu2018}, Cao et al.\ propose a framework based on DRL where actions are flexible and can be chosen by the user, and the objective of the optimization is the throughput and the handover count.
% Hence, the parameter value is not optimized directly and instead, they learn decision policy for UEs, and let UE to decide which cell to connect directly. 
In \cite{wanli2018}, Wang et al.\ propose a framework in which the UEs first are clustered based on their usage pattern and then the handover process is optimized in each cluster by a DRL method. The input to the algorithm is the RSRQ and the objectives are throughput and handover rate.
% In \cite{caolu2018}, the authors propose a framework based on DRL. This framework uses different features collected from access equipments and creates a new feature set using CNN and RNN which is sent to a policy network (a fully-connected DNN) and a decision is made for the parameter values. 
% Actions are flexible and can be chosen by the user, and the objective of the optimization is the throughput and the handover count. 
% In \cite{wanli2018} the authors propose a framework in which the UEs first are clustered based on their usage pattern. A DRL method is then used in each cluster to optimize the handover process. The input to the algorithm is the RSRQ and the objectives are throughput and handover rate. Also a supervised learning method is used to accelerate the convergence of the parameters in a newly introduced UE. 
%As it can be seen, in the above methods, the neighbors' information is not used to its full capacity and in contrast to the new models used for wireless networks, no graph is utilized for proper modeling of the network and full exploitation of the neighbors' information. Also, none of the above methods use throughput and load balancing simultaneously to ensure maximum throughput delivered to the user while preventing the stations from being over loaded.
Another newly introduced approach to the problem of handover optimization is the Contexual Bandit model which is used in \cite{infocom_dlCell} to optimize network parameters. The throughput of the cells is used as a performance metric in the reported tests. 
% Transfer learning is also used in the framework to transfer the knowledge from other cells to the subject cell.

Moreover, the use of Graph Convolutoinal Networks (GCNs)~\cite{hamilton2017, kipf2017} has also yielded significantly well-designed models to predict the network traffic and optimize the corresponding parameters. For example, in \cite{zhazha2020}, Zhang et al.\ introduce a novel handover strategy based on GCNs. The handover process is modeled as a directed graph by which the user tries to predict its future signal strength. A GCN is used to extract the underlying regularity of the best handover strategies of different users. Other works such as \cite{zhajia2020} introduce novel methods of network traffic prediction combined with a greedy search or action configuration method to optimize handover parameters. However, these existing works fail to consider the heterogeneous aspect of the cellular networks.
%In \cite{zhajia2020} the authors propose a method which uses the transition probability matrix of the handover graph to improve traffic prediction using GCN. Although the final goal of this method is traffic prediction, combined with a greedy search or action configuration method it can be used for parameter optimization.

\subsection{Motivation and Contribution}

All the above-mentioned methods solve the problem of mobility management and handover optimization to some extent. However, none of them utilizes the capacity of the neighbors' information to fully tailor the model to adapt to the special characteristics of a cellular network, where the interaction is complex and the network is heterogeneous. Also, despite the fact that these techniques consider some important measures of optimization (such as HOF rate, PP rate, throughput, load balancing, etc.), none of them approaches the problem at hand by considering two of the most important measures simultaneously (especially from the users' perspective): load balancing and throughput.
In this article, we propose an effective and efficient framework that models the network as a heterogeneous graph where we learn an implicit interaction type for each neighboring cell. Then, it incorporates the impact of neighboring cells from each interaction group in a unique way. Moreover, in contrast to the available methods in the literature, we exploit two important measures in the network to configure the parameters effectively: throughput and load balancing, which are directly related to the experience of the user in the network.

% In this article, we propose an effective and efficient framework which uses the network graph to improve information flow to the center cell. 
% This allows the subject station to be aware of the status of the neighbors which is critical while performing load balancing. 
% We utilize the graph space along with a designed embedding space to partition the neighbors into several groups and perform this task efficiently. 
% % Also, temporal grouping of neighbors' information allows aggregating larger amounts of information while avoiding further complexity in the model. 
% Moreover, in contrast to the available methods in the literature, we exploit two important measures in the network to configure the parameters effectively: throughput and load balancing, which are directly related to the experience of the user in the network. 
% % In the next section we will formulate the problem and propose our solution.



==> sections/Simu.tex <==
The experiments are conducted on a large-scale cellular network simulator constructed from real-world data. We use principal component analysis (PCA) as the mapping function $f(\cdot)$, as defined in Sec~\ref{sec:mlpmodel}, for obtaining the latent representation in the AG-GCN step. It transforms the original feature into a 2-dimensional space to perform the neighborhood augmentation and the neighbor group assignment process. The relationship operator $\gamma$ for the auto-grouping is given by Table~\ref{tab:relationshipOperator}. The permutation-invariant function $\pi$ applied on each group of neighbors is average in our experiments.

\begin{table}[t]
    \centering
    {\fontsize{8}{10}\selectfont
    \begin{tabular}{|c|c|c|}
        \hline
         $\gamma(\textbf{y}_t^{v}, \textbf{y}_t^{u})$ &  $\textbf{y}_t^{v}[0] > \textbf{y}_t^{u}[0]$ & $\textbf{y}_t^{v}[0]\leq \textbf{y}_t^{u}[0]$\\ \hline
         $\textbf{y}_t^{v}[1] \leq \textbf{y}_t^{u}[1]$ & 2 & 1 \\ 
         $\textbf{y}_t^{v}[1] > \textbf{y}_t^{u}[1]$ & 3 & 4 \\ \hline
    \end{tabular}}
    \caption{The relationship operator $\gamma$}
    \vspace{-.7cm}
    \label{tab:relationshipOperator}
\end{table}

In the following, we first introduce the used datasets along with the simulator construction. Then we discuss the learning capability of our model and compare its prediction accuracy with several benchmark models trained on the dataset.
Finally, we compare the achieved performance of different models and parameter configuration strategies based on the simulator.

\subsection{Datasets}
To perform our experiments and evaluate the proposed model, two datasets are used in this study:

\paragraph{Dataset-A:} A real metropolitan cellular network containing around 1500 cells. The collection period starts from Oct. 17 to Oct. 31, 2019, where for each day the data of cells are sampled hourly. Each data sample contains information such as the cell ID, sample time, configuration of cell parameters, and measurements of the cell states (e.g., the number of total users within the cell, the number of active users, the cell average CQI, the cell traffic load, etc.) and performance indicators (e.g., the average cell throughput, the edge user throughput, etc.). The neighbor relation information between cells are also collected and the hourly average handover counts between neighbor cells are recorded. The weekend dates are excluded since these days are not considered as rush our usage for this region of cellular networks.
	
\paragraph{Dataset-B:} Also a real metropolitan cellular network. The network contains 1459 cells, and the data is collected from Sep. 1 to Sep. 29, 2021. Each data sample contain similar information as above. 

%the samples are recorded in an hourly manner and contain important information such as cell ID, sampling time, and many of the important quantities corresponding to the performance of the cell and configuration of the network parameters (such as traffic, throughput, cell operating frequency band, etc.)
\vspace{-0.1cm}
\subsection{Reward Model Accuracy Evaluation}
In this section, we first aim to investigate how accurate our designed model can achieve in terms of predicting the system's final reward (throughput and throughput ratio) given the current network states and its corresponding handover parameter configurations.  
% {\color{blue}Chuaijie: I have moved the dataset description to the previous section, and also added how the data is simulated. I think maybe we could shorten the following part. For example, "In order to evaluate the prediction accuracy of our model, we use the simulator to generate the dataset with a random policy. On each data, the action for each cell is randomly selected within the range ..."}

\subsubsection{Dataset Generation}
In order to evaluate the prediction accuracy of our model, we use the simulator to modify Dataset-A with a random policy to diversify our network configuration. 
On each day, the A2-threshold for each cell is randomly selected around the default action -100 dBm within the range $[-105, -95]$. 
This approach provides us a fix data buffer with diverse action dataset to train all models and have a fair comparison of their accuracy. For Dataset-B, there exists a reasonable amount of the diversity in the handover parameter configuration, thus we directly use the raw dataset from the live network to perform the training and evaluation.
% \sout{This allows us to train all the models with the same dataset (a fix data buffer) and have a fair comparison of their accuracy.}

\subsubsection{Training Process and Metrics}
As samples generated by the simulator are hourly, we aggregate the samples within each day as described in Sec.~\ref{sec:mlpmodel}. In order to evaluate the model accuracy in predicting cell throughput and throughput ratio, we train the model with samples for 7 days $\{t_1,\cdots,t_7\}$.
We generate the pairs $(t_1,t_2),\cdots,(t_6,t_7)$, and train the model with these samples. 
At each day $t_i$, we sample  80\% of the data pairs from the days presented by far
%$[(t_1, t_2), \cdots,$ $(t_{i},t_{i+1})]$ 
as training and validation set, the rest 20\% serves as testing set for evaluation across different models.  We report the mean square error (MSE) to measure the reward model performance.

% {\cj{I think one of the reviewers comments is reasonable: we shuffle the data and test on past data with future data in the training set. Maybe it is better if we use the past data as training set and the next day's data as test set. Otherwise, we may need to give some justifications on this setting.}}

%\begin{figure}
%    \centering
%    \includegraphics[width=.475\textwidth]{figures/MSE_same.png}
%    \vspace{-.1cm}
%    \caption{The train and test accuracy of different models trained with the same dataset in terms of MSE.}
%    \vspace{-.2cm}
%    \label{fig:ModelsMSEsame}
%\end{figure}

% the samples $(t_1, t_2), \cdots, (t_{i},t_{i+1})$ are shuffled and 80\% of them are used for training, validation and the rest for testing. We report the mean square error (MSE) to measure the reward model performance.
% \begin{equation}
%     {\rm MSE}^i_1 = \frac{1}{t_i}\sum_{t=2}^{t_i}\frac{1}{N_t}\sum_{j=1}^{N_t} (\hat{\alpha}_{t}^{j}-\alpha_{t}^{j})^2,
% \end{equation}
% and
% \begin{equation}
%     {\rm MSE}^i_2 = \frac{1}{t_i}\sum_{t=2}^{t_i}\frac{1}{N_t}\sum_{j=1}^{N_t} (\hat{\beta}_{t}^{j}-\beta_{t}^{j})^2.
% \end{equation}
% In Fig.~\ref{fig:thrpMSE} and Fig.~\ref{fig:ratioMSE} we compare the predicted throughput ratio and cell throughput and with the actual ones, respectively.
% In these figures the zero error is interpreted as the straight line shown in figures.
% As seen for both objectives, the predictions are mostly around the indicator line meaning an acceptable accuracy of the model.

% \begin{figure}
%     \vspace{-.5cm}
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/CriticModel.png}
%     \vspace{-.5cm}
%     \caption{Accuracy of the cell throughput ratio model by comparing the predicted and true values of the validation set.}
%     \label{fig:thrpMSE}
% \end{figure}
% \begin{figure}
%     \vspace{-.5cm}
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/NewCriticModel.png}
%     \vspace{-.5cm}
%     \caption{Accuracy of the throughput model by comparing the predicted and true values of the validation set.}
%     \label{fig:ratioMSE}
% \end{figure}


\begin{figure}
    \vspace{-.5cm}
    \subfloat[][]{\includegraphics[width=.235\textwidth]{figures/TestMSE_old_data_thrp.pdf}}
	\subfloat[][]{\includegraphics[width=.23\textwidth]{figures/TestMSE_new_data_thrp.pdf}}
    % \includegraphics[width=.475\textwidth]{figures/TestMSE_old_data.pdf}
	\vspace{-.45cm}
	\caption{Mean squared error of the throughput for test data of (a) Dataset-A and (b) Dataset-B for TAG-GCN.}
	\vspace{-.6cm}
	\label{fig:TAG-GCN_test_mse_thrp}
\end{figure}

% \begin{figure}
%     \vspace{-.2cm}
%     \includegraphics[width=.475\textwidth]{figures/TestMSE_new_data.pdf}
% 	\vspace{-.8cm}
% 	\caption{Mean squared error of the (a) throughput and (b) throughput ratio models for TAG-GCN on the test data for Dataset-B.}
% 	\vspace{-.5cm}
% 	\label{fig:TAG-GCN_new_test_mse}
% \end{figure}

\subsubsection{Comparison with Benchmark Models}\label{sec:benchmark}
%\yx{Need a bit justification why we do not use any existing works instead of create our own baselines. 1) Data driven approach 2) }
% {\color{magenta}
% \sout{First of all, we want to address our choice with the comparison baselines. Because of the uniqueness of our problem, existing solutions for optimizing handover parameters are either not appropriate or no apparent way how to directly adapt to our problem. We provide the following reasons. Traditional handover optimization methods rely on designing fuzzy rules based on different measures of the QoS in the network~\cite{vasmah2012}, however, designing proper rules is complex and cannot handle the change of system dynamic well. Instead, we hope to use a data-driven approach. Among the data-driven approaches, the (deep) RL method gains the most attention~\cite{caolu2018,wanli2018}. However, in our problem, the network provider will only allow exploring the parameter values within a limited time window and allow changing action one time every day to make sure the stability of the network system. Thus, we only have limited days (around 10 days) for exploration the best action and RL models usually need longer episodes to optimize the accumulated return. We did some preliminary attempt to adapt the RL paradigm from the literature into our problem, however, it does not show advantages over our simpler design, as demonstrated in Appendix Sec.~\ref{sec:appendix_rl}.}}

{It is important to note that, because of the uniqueness of our problem, existing solutions for optimizing handover parameters are either not appropriate to solve it or there is no apparent way to directly adapt them to our problem. For instance, traditional handover optimization methods rely on designing fuzzy rules based on different measures of QoS in the network~\cite{vasmah2012}, however, designing proper rules is complex and cannot handle the change in highly dynamic systems well. Instead, we hope to use a data-driven approach, among which the (deep) RL method gains the most attention ~\cite{caolu2018,wanli2018}. However, in this type of problems, the network provider will only allow limited exploration of the parameter values (e.g., allow changing the A2 value once a day) to ensure the stability of the network. Thus, we only have limited days (around 10
days) for exploring the best action. RL models, nevertheless, usually need longer episodes to optimize the accumulated return. Despite this fact, we made some preliminary attempt to adapt the RL paradigm from the literature into our problem which did not show any advantage over our simpler design as demonstrated in Appendix Sec.~\ref{sec:appendix_rl}.}

In order to show the effectiveness of our proposed reward model, we compare it with alternative designs for the prediction model.
In Appendix Table \ref{tab:Models}, we summarize our benchmarks and the properties of each model.
The first model is MLP, where we only use the features of the center cells and ignore the neighboring cells' features.
In GCN model, we follow the typical GCN formulation~\cite{hamilton2017} and process the network as a homogeneous graph where the neighbor information is aggregated jointly without distinction. The AG-GCN model ignores the temporal dependencies of the data which we consider in our proposed TAG-GCN model.
In Fig.~\ref{fig:TAG-GCN_test_mse_thrp}, we compare the prediction accuracy of these models for throughput prediction in Dataset-A and B. 
% {For this purpose, we use Dataset-A and, also, to make a meaningful comparison, we assign random values to the action parameter to make the available data to all models identical.} 
We observe the best accuracy for the test set is achieved by TAG-GCN, indicating that our neighbor aggregation and temporal features extraction have a considerable impact on the reward modeling for cellular networks. The same test is performed throughput ratio and included in Appendix Sec.~\ref{sec:appendix_mse}
% and the results are presented in Fig.~\ref{fig:TAG-GCN_new_test_mse}. Note that, in this case, despite all the fluctuations of the resulting mean squared error value, our proposed model still outperforms the rest of the models.}
% \sout{Note that, for the throughput model, the error increases in the third day (2019-10-21) since only one pair of data is available to train the model (2019-10-17,2019-10-18) and the error decreases as more data becomes available.}

% {\cj{1. The sentence "we assign random values to the action parameter which are identical among the models", does it mean that they are using the same random data set? 2. For the same day, are all models using the same training and test sets? 3. Maybe need to add a few words on why weekends are excluded in the results.}}

% \sout{\mm{In order to verify the effectiveness of our model in the real-world data, we compare the modeling accuracy of different models on Dataset-B in Fig.~\ref{fig:TAG-GCN_new_test_mse}}}

%\begin{table}
%	\centering
%	{\fontsize{8}{15}\selectfont
%	\begin{tabular}{|c|c|c|c|c|}
%		\hline
%		Time & EGNA & Rule-based & KMeans & GCN \\
%		\hline
%		10-22 & 0.017$\pm$0.001 & 0.016$\pm$0.001 & 0.016$\pm$0.002 & \\
%		\hline
%		10-23 & 0.015$\pm$0.002 & 0.015$\pm$0.001 & 0.014$\pm$0.001 & \\
%		\hline
%		10-24 & 0.014$\pm$0.001 & 0.014$\pm$0.002 & 0.015$\pm$0.002 & \\
%		\hline
%		10-25 & 0.012$\pm$0.001 & 0.013$\pm$0.001 & 0.012$\pm$0.001 & \\
%		\hline
%	\end{tabular}
%    }
%	\caption{Average and standard deviation of the mean squared error values on the testing data for the last four days for different neighbor grouping schemes.}
%	\label{tab:AG_val_mse}
%\end{table}

%\begin{table}
%	\centering
%	{\fontsize{8}{15}\selectfont
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			Time & EGNA & Rule-based & KMeans & KMeans2D \\
%			\hline
%			10-22 & 0.017$\pm$0.001 & 0.016$\pm$0.001 & 0.016$\pm$0.002 & 0.020$\pm$0.003 \\
%			\hline
%			10-23 & 0.015$\pm$0.002 & 0.015$\pm$0.001 & 0.014$\pm$0.001 & 0.014$\pm$0.001 \\
%			\hline
%			10-24 & 0.014$\pm$0.001 & 0.014$\pm$0.002 & 0.015$\pm$0.002 & 0.015$\pm$0.002 \\
%			\hline
%			10-25 & 0.012$\pm$0.001 & 0.013$\pm$0.001 & 0.012$\pm$0.001 & 0.012$\pm$0.001 \\
%			\hline
%		\end{tabular}
%	}
%	\caption{Average and standard deviation of the mean squared error values on the testing data for the last four days for different neighbor grouping schemes.}
%	\label{tab:AG_val_mse}
%\end{table}

%Also, Table~\ref{tab:AG_val_mse} shows the average and standard deviation of the mean squared error values on the testing data for the last four days using the above mentioned schemes.???


% In the following we compare the accuracy of the presented models in terms of the MSE under two distinct scenarios.
% In Fig.~\ref{fig:ModelsMSEsame}, we compare the prediction accuracy of the models where instead of using the recommended actions by the models at each day and change the states of the next day accordingly, we use the same set of random actions for all models in each day.
% Since the actions are the same for all the models, they have the same states and hence they all trained by the same generated dataset and we can have a fair comparison between the models accuracy.
% In Fig.~\ref{fig:ModelsMSE}, we use the recommended actions of the models and the states achieved by them to train the models.
% Thus, the models are trained by different datasets achieved based on their recommendations instead of random actions in the previous case.


% \begin{figure}[]
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/MSE-new.png}
%     \caption{The train and test accuracy of different models trained based on their recommended actions in terms of MSE.}
%     \label{fig:ModelsMSE}
% \end{figure}

\vspace{-5pt}
\subsection{Overall Optimization Performance}
\subsubsection{The Action Recommendation Process}
In the following experiments we use the presented models to recommend the actions for Dataset-A.
The actions in day $t_1$, i.e., Oct. 17, has been set to the default action which is -100~dBm.
% For the second day, i.e., October 18, three distinct types of action initialization are used, including random, negative slope, and expert's rule initialization.
Unless otherwise stated, the action for the second day, i.e., Oct. 18, is initialized by a set of random actions around the default action in the range of $[-105, -95]$.
The model is trained iteratively in each day and used to recommend actions for the next day.
% We use the simulated data generated under the previous actions to train the models and recommend actions for day $t_3$ and continue this procedure until the last day.
The process is depicted in Fig.~\ref{fig:training}, where states of the cells at day $t_i$ are given to the trained model to predict performance metrics of the network at day $t_{i+1}$ and the action $a^v_{t_i}$ is adjusted for each cell based on the reward predictions.
Finally, the network states and performance measurements for day $t_{i+1}$ are computed by the cellular network simulator and used for model training and action recommendation in the following day.


% are initialized by the user to get the states of cells in day $t_2$.
% Then the training process starts from day $t_2$, where the model is trained by $(t_1,t_2)$ samples and given the trained model and the states of cells at day $t_2$, the actions are tuned to optimize the throughput ratio and cell throughput.

% Finally, at day $t_7$, the model is trained by all the previous sample pairs and recommend actions for day $t_7$ to optimize the objectives of next 4 days.
% The training process is shown in 
% At each day $t_i$, $i<7$, the sample pairs $(t_1,t_2),...,(t_{i-1},t_i)$ 

% The dataset we use in our experiments is collected from base stations of a metropolitan cellular network containing more than 1400 cells.
% The data is collected for 11 days starting from October 17 to October 31, 2019, where for each day the data of cells are sampled hourly.
% Each data sample contains information such as the cell ID, sample time, configuration of different parameters, cell state measurements and performance measurement of the cell.
% These measurements includes information such as the number of total users within the cell, the number of active users, the average CQI of the cell, the average data traffic, and the occupied bandwidth. 

% The states of the cells are either fixed or variable. 
% Those fixed states such as CQI are not affected by tuning the action and thus are directly used from the dataset based on the real network.
% The variable states such the throughput are highly dependent on the action.
% Consequently, we use a simulator that can precisely mimic the real environment for cellular network to compute the performance measurements after changing the action.
% Finally the fixed states of the dataset along with the computed measurements based on the simulator are merged together to train the model and tune the action for the next day.

% In order to train the throughput ratio and cell throughput models, we define two categories of cellular network state measurements, cell-based and cluster-based states.
% The cell-based states are defined for each single cell without considering its neighborhood.
% On the other hand, the cluster-based state measurements are defined for each cluster and 
% computed as the ratio of the center cell measurements to the average of that feature in the cluster. 
% Let us assume that $\pi^v_t$ is one of the states of the center cell $v$ at day $t$, then the cluster-based state $\Pi^v_t$ is defined as
% \begin{equation}
%     \Pi_t^v = \frac{\pi^v_t}{\frac{1}{|{\cal N}(v)|}\sum_{u\in{\cal N}(v)}\pi^u_t}.
% \end{equation}
% For our experiments, we feed the throughput ratio and cell throughput models with only the cluster-based and cell-based state measurements, respectively. 


% \subsection{Training Process and Model Accuracy}
% {\color{blue}Chuaijie: based on our last discussion, I think the model accuracy should be evaluated on the randomly generated dataset. So no action recommendation is involved here. Probably the iterative training and recommendation procedures should be moved before the "Overall performance" part.}


% Cell state data are first preprocessed. 
% In order to improve the robustness of the model we select only the busy hours $h$ for each single day, where $h\in[9,22]$.
% Moreover, we remove the samples with low traffic indicator to further challenge the model learning capability.
% For each objective in our model, we choose the most related state features to that objective.
% Then before the training we normalize the state vector to speed up the training process. 


% \subsection{Benchmark Models}


\subsubsection{Baseline Performance Bounds}
In addition to the result achieved by the actions recommended by the models, we use three baseline performance bounds achieved by the default A2-threshold, the expert rule, and the optimal actions of the simulator.
As stated before the default A2-threshold value is $-100$~dBm and this is used as the lower bound in the following experiments.
The optimal actions in the simulator are obtained by brute-force search and it introduces the upper performance bound. 
The expert rule-based action recommendation is a simple rule presented in (\ref{eq:experts}).
The performance achieved by the expert rule is better compared to the default action.
However, there is still a big gap to the throughput achieved by the optimal actions given by the simulator. 
% and in the following experiments we show how much we can reduce this gap by our algorithm. 

% \subsection{Action Distribution}
% The action exploration in TAG-GCN model is performed by the proposed algorithm presented in the previous section, where one action is recommended per day for each cell.
% The actions are chosen to configure the A2-threshold-RSRP parameter which is in the range of $[-112,-93]$ dBm in the cellular network.
% In Fig.~\ref{fig:ActionDist}, the distribution of the recommended actions for the final day in our experiment is illustrated. 
% As seen our action exploration strategy can recommend actions in a wide range and it is not biased.

% \begin{figure}[t]
%     \vspace{-.4cm}
%     \centering
%     \includegraphics[width=.5\textwidth]{figures/0_INTERFREQHOGROUP_INTERFREQHOA2THDRSRP_jan19}
%     \caption{Recommended action distribution for the final day of experiment.}
%     \label{fig:ActionDist}
% \end{figure}

\begin{figure}[t!]
    \centering
    \vspace{-.3cm}
    \includegraphics[width=.45\textwidth]{figures/trainingProcess.pdf}
    \vspace{-.5cm}
    \caption{The process of action recommendation by the trained model and the simulator.}
    \vspace{-.6cm}
    \label{fig:training}
\end{figure}

\begin{figure}
    \vspace{-.1cm}
    \centering
    \includegraphics[width=.475\textwidth]{figures/reward_total.pdf}
    \vspace{-.8cm}
    \caption{Performance comparison of different models along with Best Action curve initialized with random actions. The lower left part is a zoomed-in version of the curves on the right.}
    \vspace{-.45cm}
    \label{fig:ModelPerformance}
\end{figure}

\subsubsection{Results}
In the following experiments, we compare the performance of the network under the actions recommended by different models in terms of the network throughput as defined in eq~(\ref{eq:throughput}). We plot the trajectory of the throughput difference to the default A2-threshold baseline (dash black line) in Fig.~\ref{fig:ModelPerformance}. 
% We compare the overall performance of the cellular network in terms of the network throughput for all the models listed in Table~\ref{tab:Models}.
We repeat all the experiments 20 times for all models, where each run uses the same set of random actions on the first action exploration day (Oct. 18) for all the models.
We also show the performance achieved through the expert rule action recommendation, default action, and the best actions of the simulator (random actions are also used on Oct. 18 for the curve of the Best Action). The quantitative results for Fig.~\ref{fig:ModelPerformance} and are summarized in Tables~\ref{tab:num_res_diff_models} in Appendix. 
TAG-GCN can achieve significantly better average throughput in the final days and also converges faster than the alternatives. This indicates the importance of our auto-grouping GCN design to tailor the heterogeneous property of the cellular networks.
%It should be noted that the TAG-GCN model has the lowest variance in the achieved performance showing its stability in the parameter configuration process.
Besides, as expected, all the learning-based models can beat the expert rule algorithm which is highly dependent on human experience and is unable to recover from the performance degradation caused by a bad random initialization on the first day. Furthermore, to show the effectiveness of our proposed model in terms of load balancing and enhancing the throughput ratio in a cluster, we illustrate the progress of the throughput ratio for some selected cells in Fig.\ref{fig:cell_thrp_ratio_progress}. As it can be seen, the throughput ratio of the clusters form a trajectory that converges to 1 which is the ideal target value.

\subsubsection{Ablation Studies}
\textbf{1) The multi-objective action recommendation strategy}
In Appendix section~\ref{sec:appendix_multi_obj} Fig.~\ref{fig:Multi_objPerformance}, we show an ablation study on the effectiveness of our proposed multi-objective action recommendation strategy. Our proposed TAG-GCN model with both load-balancing and throughput as optimization objectives can outperform others single objective alternatives, achieving the best average throughput in the final days across random trials.


% For each setting, we repeat our experiment five times with TAG-GCN as the reward model but follow different action configuration strategies. Other than the multi-object formulation, we consider two alternatives for action configuration, one by considering only the cell throughput in the optimization problem, and one by considering only the load-balancing objective.
% As shown in Fig.~\ref{fig:Multi_objPerformance}, our proposed TAG-GCN model with both load-balancing and throughput as optimization objectives can outperform others, achieving the best average throughput in the final days across random trials. The quantitative results for Fig.~\ref{fig:Multi_objPerformance} is summarized in Appendix tables~ \ref{tab:num_res_diff_opt}.


\begin{figure}
% 	\vspace{.4cm}
	\centering
	\includegraphics[width=.475\textwidth]{figures/thrpt_ratio_progress.pdf}
	\vspace{-.7cm}
	\caption{Trend of the throughput ratio value for sample clusters.}
	\vspace{-.6cm}
	\label{fig:cell_thrp_ratio_progress}
\end{figure}

% The quantitative results for Fig.~\ref{fig:ModelPerformance} and Fig.~\ref{fig:Multi_objPerformance} are summarized in Tables~\ref{tab:num_res_diff_models} and \ref{tab:num_res_diff_opt}, respectively. 
% We present the achieved network throughput by different models divided by the performance achieved by the best actions of the simulator for the last 4 days of the experiments. 
% As seen, in the first table the proposed method is outperforming the rest of the methods and yields better average throughput. {Furthermore, our method also yields lower variance with respect to change in the initial values of the actions, which is a significant advantage. In general, our method proves to be very robust in this regard.} 
% The second table demonstrates the effectiveness of the multi-objective optimization strategy. 
% In this table, we have denoted three different variants of TAG-GCN which represent three optimization strategies, namely, multi-objective strategy using both throughput and throughput ratio models (TAG-GCN1), single objective strategies using throughput ratio (TAG-GCN2), and throughput models (TAG-GCN3). As the res:appults in the table show, the multi-objective strategy outperforms the single objective ones and therefore is superior.

\textbf{2) Different action initialization schemes}
Besides, in Appendix section~\ref{sec:appendix_init}, we present an ablation study on the different initialization schemes on the first action exploration day. We can observe that regardless of the type of initialization, our design can quickly converge to the desired model performance even without strong prior information from the network.
\vspace{-5pt}

% our design can converge to almost the same performance in the final days, which indicates that even without strong prior information from the network, our design can still quickly converge to the desired model performance.
% In Fig.~\ref{fig:Multi_objPerformance}, we show an ablation study on the effectiveness of our proposed multi-objective action recommendation strategy.
% We repeat our experiment 5 times with TAG-GCN as reward model. initialized with random actions at day $t_2$ but follow different action configuration strategies.
% As demonstrated in Sec.~\ref{sec:opt} we propose a novel action configuration strategy by optimizing the load balancing in each cluster and also keeping the throughput of each cell as high as possible.
% Here we consider two more approaches for action configuration, one by considering only the cell throughput in the optimization problem, and one by considering only the load-balancing.
% As shown in the figure, our proposed TAG-GCN model with both load-balancing and throughput can outperform others and at the same time have the lowest variance in the achieved result.

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.475\textwidth]{figures/opt.pdf}
%     \vspace{-.8cm}
%     \caption{The impact of different optimization objectives for the parameter configuration in our proposed TAG-GCN model.}
%     \vspace{-.3cm}
%     \label{fig:Multi_objPerformance}
% \end{figure}

% In Fig.~\ref{fig:thrpRatio}, we study the impact of our approach on network load balancing and compare it with different models. The average throughput ratio across all clusters is shown for each day.
% As shown in the figure, as we approach the final days, the average throughput ratio using our method moves toward the value of an ideally balanced network (in which this ratio must be equal to 1) and outperforms the rest of the methods in this regard. Notice the degradation in throughput ratio during earlier days. This comes from the non-stationary network change (a similar trend is seen in the default baseline) as well as the poor reward model due to the limited training labels in the early days.

% In Fig.~\ref{fig:thrpRatio}, we study the impact of our approach on network load balancing metric and compare it with the performance with default action.
% The average throughput ratio of different clusters is shown for all days.
% As seen, as we reach the final days, the average throughput ratio of our approach keeps decreasing and it achieves smaller distance to one which shows its effectiveness.

% This load balancing by our model can highly affect the action configuration and performance of the network as shown in the previous figures.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.475\textwidth]{figures/thrp_ratio_avg.pdf}
%     \vspace{-.6cm}
%     \caption{The impact of TAG-GCN model on the load balancing measured as the average throughput ratio across the network.}
%     \vspace{-.6cm}
%     \label{fig:thrpRatio}
% \end{figure}


==> sections/TAG_GCN.tex <==
%Address the difficulties of this problem and give a motivation why we use our designed framework.
In this section, we present our data-driven solution to learn an accurate reward model to imitate how the network will respond to given networks' states and handover parameter (A2-threshold) configurations, which we will intertwine with the term action throughout this paper. As stated in Sec.~\ref{sec:problemFormulate}, we aim to have this reward model that can accurately predict the cell performance metrics such as throughput and throughput ratio, which will be a determining factor during our action configuration stage.

In the following, we introduce three key components of our method. \textit{First}, to better capture the dependency between each cell and its neighboring cells, we introduce our novel method for neighboring cell feature aggregation. \textit{Second}, we propose a temporal feature aggregation step with Recurrent Neural Networks (RNN) to model the temporal correlation from the historical sequence of the network states. \textit{Third}, we elaborate the overall training process, considering the impact from the neighboring cells, the temporal correlation in the network states and the action we aim to optimize. 


\subsection{Auto-Grouping GCN for Neighbor Aggregation}

Since the handover parameters heavily impact the learning problem on the graph of the center cells as well as the neighboring cells, we aim to capture the neighboring cell information during our modeling process. Recently, message-passing neural networks (MPNNs) in the form of graph neural networks (GNN) have been introduced and demonstrated to be effective in modeling real world applications with structure information. The dependencies in the data set are modeled using a graph \cite{kipf2017,hamilton2017, ying2018,NGCF_wang19}. In each layer of a graph neural network, each node's representation includes the features from itself as well as the features from its neighboring nodes (messages sent from the neighborhood). We believe the graph neural network framework is suitable for handling the dependencies between the center cell and the neighboring cells in cellular networks.  We first elaborate on how we transfer the cellular network modeling problem into a learning problem on a graph. Then we delve into the challenge of using the message passing framework in cellular networks.

\subsubsection{Graph-Based Cellular Network Modeling}

We construct a graph ${\mathcal G}_t=(\mathcal{V}_t,\mathcal{E}_t, \mathbf{X}_t)$ for day $t$, where each node $v\in \mathcal{V}_t$ represents one cell and is associated with a feature vector $\textbf{x}_t^{v}\in\mathbb{R}^d$ ($v$-th column of $\mathbf{X}_t\in\mathbb{R}^{d\times |\mathcal{V}_t|}$), including the statistical properties of node $v$ measured on day $t$. 
The statistical properties could include the antenna transmission power, physical resource block (PRB) usage ratio, the amount of data traffic, and the transmission bandwidth. These features serve as the node attributes. The edge set $\mathcal{E}_t$ encodes the interactions between cells based on the handover events between pairs of cells. Based on historical data, if any pair of cells has an average number of handover events above a threshold $\tau$, we assume an edge between those two cells. The neighboring set for node $v$ is denoted as $\mathcal{N}_t^g(v)=\{u|u\in \mathcal{V}_t,(u,v)\in \mathcal{E}_t\}$. 

Successful applications of graph neural networks mostly rely on a homogeneous graph structure. For example, in social networks or recommendation systems, each edge represents a positive correlation between the adjacent nodes~\cite{kipf2017, fan2019graph}. The message passing framework applies the same transformation function to every neighbor and aggregates across them to obtain the neighbor representation, as shown in Fig.~\ref{fig:normal_gcn}. There is a rich literature that studies how to process a heterogeneous graph with multiple relation types~\cite{schlichtkrull2018modeling, zhang2019heterogeneous}. Those works are established on the prior knowledge of the given relation type between each pair of nodes and then use a meta-path design to distinguish the information coming from different types of neighbors. Such an approach is not applicable to our problem. 

\begin{figure}
    \vspace{-.3cm}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/regulargcn.pdf}
    \vspace{-.7cm}
    \caption{Commonly used Graph Neural Network design.}
    \vspace{-.75cm}
    \label{fig:normal_gcn}
\end{figure}

When using a graph to represent the interactions between cells in cellular networks, we are unaware of the interaction types. Due to the heterogeneous nature of the cellular network, the relationships between the neighboring cells can be complex. 
% For example, for the transmission power feature, the adjacent cells might have a negative correlation. But on the traffic user feature, the adjacent cells might have a positive correlation. 
Concretely, there might be an implicit $M$ latent relationship types $\mathcal{R} = \{r_1,r_2, \cdots ,r_M\}$ that can be learned to better handle the complex interactions in the cellular networks. Intuitively, assuming each cell is represented by its states such as PRB usage, channel quality indicator (CQI), the amount of traffic, and available bandwidth, after dividing the neighbors into different groups, we would hope the neighbors in each group have similar network states with respect to the center cell to better capture the rich information from neighboring cells in a distinguishable way. 
Thus, inspired by the above motivation and a recent work~\cite{pei2019geom}, we propose a novel GCN approach called Auto-grouping GCN (AG-GCN) to characterize this special property of cellular networks when handling the interactions between the neighboring cells. In the following subsection, we elaborate upon the detailed steps to realize our AG-GCN design. 

%\begin{figure}
%    \centering
%    \includegraphics[width=.5\textwidth]{figures/AG-gcn.pdf}
%    \vspace{-.3cm}
%    \caption{The structure of the AG-GCN neighbor aggregation. The number of selected neighbors in the Euclidean space is determined by the number of neighbors in the graph space.}
%    \label{fig:nei_aug}
%\end{figure}

\subsubsection{Neighborhood Augmentation} \label{sec:neighbor_aug}
%Define motivation why we need neighborhood augmentation
In cellular network modeling, only a limited amount of experiment budget is allowed by network operators. We will not have enough diverse historical data (state-action pairs) to train our data-driven model. Besides, since we construct the graph based on the handover events, there are cells that have a very limited number of neighboring cells. Thus, in our design, we use a data augmentation technique in the form of neighbor cell augmentation to enrich the features of each cell. The neighbor cell augmentation is based on the similarity between cells in a latent space. 

%  $\textbf{x}_t^v$
We define a feature transformation function $f(\cdot) : \mathbb{R}^d \rightarrow \mathbb{R}^l$ which maps the input node feature  $\textbf{x}_t^v \in\mathbb{R}^d$ to a latent space $\textbf{y}_t^{v}\in\mathbb{R}^l$, where $\textbf{y}_t^{v} = f(\textbf{x}_t^{v})$.
In order to capture the long-range dependencies and similarity in the cellular network, we design an additional neighborhood in the latent representation space based on Euclidean distance. For each node $v\in \mathcal{V}_t$, we form the augmented neighborhood ${\mathcal N}_t(v)=\mathcal{N}_t^g(v)\cup \mathcal{N}_t^s(v)$, where $\mathcal{N}_t^g(v)$ and $\mathcal{N}_t^s(v)$ are the neighbors of node $v$ in the original graph and in the latent space, respectively.
The neighbors in the latent space are selected based on their Euclidean distance to the center cell. The $n$ nearest nodes in the latent space are selected to create neighborhood $\mathcal{N}_t^s(v)$ for cell $v$, where the number of nodes we select based on the feature similarity is equal to the neighborhood size in the original graph $|\mathcal{N}_t^g(v)|=|\mathcal{N}_t^s(v)|=n$. The neighbor augmentation module in Fig. \ref{fig:nei_aug_aut_grp} illustrates this process.

%\begin{figure}
%	\centering
%	\includegraphics[width=.4\textwidth]{figures/auto_grouping.pdf}
%	\vspace{-.3cm}
%	\caption{Constructing $ M $ groups of neighbors using the augmented neighbors' set (demo example for $l=2$ and $|\mathcal{R}|=4$). Empty groups are filled with zeros.}
%	\label{fig:auto-grouping}
%\end{figure}

\begin{figure*}
    \vspace{-.3cm}
	\centering
	\includegraphics[width=1\textwidth]{figures/TAG_GCN_Structure_v2.pdf}
	\vspace{-.8cm}
	\caption{The flow of information from graph structure to final prediction. This flow path is used to form the training pipeline of two models for predicting the throughput $\hat{\alpha}$ and the throughput ratio $\hat{\beta}$ for $\mathcal{T}_{in}=\{1,2,\cdots,t-1\}$. In the neighbor augmentation module, the number of selected neighbors in the Euclidean space is determined by the number of neighbors in the graph space. The auto-grouping module constructs $M$ groups of neighbors by using the augmented neighbors set (demo example for $l=2$ and $|\mathcal{R}|=4$). Empty groups are filled with zeros.}
	\label{fig:nei_aug_aut_grp}
	\vspace{-.4cm}
\end{figure*}

\subsubsection{Neighborhood Auto-Grouping}
% The final step of our AG-GCN method, is the auto-group neighbor aggregation.
Once we have obtained the augmented neighborhood set, the neighbors in the augmented neighborhood ${\mathcal N}_t(v)$ are divided into different groups by a geometric operator $\gamma$.
Consider node $v$ and its neighbor node $u\in{\mathcal N}_t(v)$. The relation between them on day $t$ is denoted as $\gamma(\textbf{y}_t^{v}, \textbf{y}_t^{u}) : (\mathbb{R}^l, \mathbb{R}^l) \rightarrow \mathcal{R}=\{r_1,r_2,\cdots,r_M\}$. Intuitively, we aim to assign an interaction type (edge membership) between each pair of center and neighbor cell based on their latent representations. 
For each group $r_i\in\mathcal{R}$, the neighborhood feature set at time $t$ is defined as:
% $\gamma$ essentially group the neighbors of cell $v$ at day $t$ as 
\begin{equation}
    \mathcal{N}_t^{r_i}(v) = \{u|u\in{\mathcal N}_t(v), \gamma(\textbf{y}_t^v,\textbf{y}_t^u)=r_i\}.
\end{equation}
% $\mathcal{R} = {r_1,r_2,….,r_M}$
The auto-grouping module in Fig. \ref{fig:nei_aug_aut_grp} demonstrates this process. Note that yellow neighbors (marked with *) are the projected counterparts of the neighbors in the graph space, while the green neighbors (marked with +) correspond to the augmented neighbors from the Euclidean space.

\subsubsection{Conditional Message Passing}
Since the order within each neighbor group should not impact the output of the representation, we apply a permutation invariant function $\pi(\cdot)$ on the neighbors within each group (mean pooling across each feature dimension) and aggregate them separately.
Fig.~\ref{fig:nei_aug_aut_grp} shows an example of the AG-GCN, where $l=2$ and $|\mathcal{R}|=4$ and the representation after the permutation invariant function $\pi(\cdot)$ is shown by black dashed arrows ended to nodes 1, 2, 3, and 4.
Then for each group $r_i\in\mathcal{R}$, a  non-linear transform is further applied as:
\vspace{-0.1cm}
\begin{equation}
    \textbf{z}_t^{v,r_i} = \sigma\Big(\textbf{W}_t^{v,r_i}\cdot\pi\big(\{\textbf{x}_t^u|u\in  \mathcal{N}_t^{r_i}(v)\}\big)\Big),
\end{equation}
\vspace{-0.1cm}
where $\textbf{W}_t^{v,r_i}$ is a learnable weight matrix for the neighbors in group $r_i$ of node $v$ at day $t$, and $\sigma(\cdot)$ is a non-linear function, e.g., $\tanh$. 
Then for each node we aim to aggregate the transformed neighborhood features from their different groups of neighbors in a distinguishable way. The vectors $\textbf{z}_t^{v,r_i}$ for $r \in \mathcal{R}$ are further aggregated by a concatenation operation:
%function $\omega(\cdot)$ as
% \begin{equation}\label{eq:neighbor_input}
%     \textbf{h}_t^v = \mathop{\omega}_{r \in \mathcal{R}} (\textbf{z}_t^{v,r}).
% \end{equation}
\vspace{-0.1cm}
\begin{equation}\label{eq:neighbor_input}
    % \textbf{h}_t^v = \omega([\textbf{z}_t^{v,r_1}; \textbf{z}_t^{v,r_2}; \dots; \textbf{z}_t^{v,r_M} ]),
    \textbf{h}_t^v = [\textbf{z}_t^{v,r_1}; \textbf{z}_t^{v,r_2}; \dots; \textbf{z}_t^{v,r_M} ],
\end{equation}
where $[\,\,;\,]$ represents concatenation.




% Then, we apply a permutation invariant function $\pi(\cdot)$ on the neighbors of all each group and aggregate them separately.
% This procedure for the case of $R=4$, is shown by black dashed arrows ended to nodes 1, 2, 3, and 4 in Fig.~\ref{fig:gcnmodel}.
% It should be noted that when there is no neighbor in group $r$ of the center cell $v$, i.e. $\mathcal{N}_r(v)=\emptyset$, a vector of all zeros with the same size as other groups is assigned to group~$r$.
% Then for $r\in\{1,2,\cdots,R\}$, a multiple layer perceptron (MLP) model is trained for each group of neighbors to apply the following non-linear transform
% \begin{equation}
%     \textbf{z}_t^{v,r} = \sigma\Big(\textbf{W}_t^{v,r}\cdot\pi\big(\{\textbf{x}_t^u|u\in \mathcal{N}_r(v)\}\big)\Big),
% \end{equation}
% where $\textbf{W}_t^{v,r}$ is a learnable weight matrix for the neighbors in group $r$ of node $v$ at day $t$, and $\sigma(\cdot)$ is a non-linear function, e.g., $\tanh$. 
% The last step in the auto-grouping neighbor aggregation is to aggregate the transformed features of different groups of neighbors at the center cell in a distinguishable way where the outputs of the MLPs are further aggregated by function $\omega(\cdot)$ as
% \begin{equation}\label{eq:neighbor_input}
%     \textbf{h}_t^v = \omega(\textbf{z}_t^{v,r},r), \text{~~for $r\in\{1,2,3,4\}$}.
% \end{equation}
% This function takes an ordered object as the input to distinguish the features from different groups to explicitly extract the information of the structural neighborhood.

% This neighborhood grouping helps us to avoid information loss.
% The regular GCN methods only adopt a permutation-invariant function such as average to aggregate the neighbors information and thus, lose too much information.
% On the other hand, considering all the neighbors directly, dramatically increases the time and space complexity of the model, which is almost impossible due to the limited resources.
% Consequently, our solution is to balance this trade-off between the performance and the model simplicity by grouping the neighbors.
% As seen, our grouping strategy, divides the neighbors into several groups based on their features with respect to the center cell and then apply a permutation-invariant function on each single group.
% This approach helps us to keep more information without huge load of model complexity.
% Assuming each cell is represented by its states such as physical resource block (PRB) usage, channel quality indicator (CQI), traffic amount, and available bandwidth. After grouping the neighbors into different groups, the neighbors in each group will have similar PRB usage, CQI, traffic amount, and available bandwidth with respect to the center cell.

\subsection{Temporal Feature Modeling}
Capturing the trend in the evolution of the states of each cell within a day properly can benefit the prediction of the performance metric for the following day.  We propose to use additional temporal features for each center cell to extract the changing dynamic pattern of its states within each day to further improve the reward model performance.
We assume the samples of the center cell $v$ at day $t$ can be divided into $K$ groups by their temporal order. For all the samples in each group $k$, we take the average network state for each group of samples and denote it as $\textbf{x}_{t,k}^{v}$. We use an RNN layer to capture this temporal dependency of the features from different groups by feeding all the network states as an input sequence $\textbf{P}_t^{v} = \big[{\textbf{x}_{t,1}^{v}}^T; {\textbf{x}_{t,2}^{v}}^T; \cdots; {\textbf{x}_{t,K}^{v}}^T\big]^T\in\mathbb{R}^{K\times d}.$     
The output of the temporal feature modeling phase can be written as:
\begin{equation}
    \textbf{c}_t^{v} = {\rm RNN}(\textbf{P}_t^{v}, \delta) \in \mathbb{R}^{d'},
\end{equation}
where $\delta$ is the set of trainable parameters of the RNN layer, and $d'$ is the output dimension of the RNN layer. 

\subsection{Overall Training Pipeline}
The main purpose of the model is to estimate the real network‘s response, and predict the throughput ratio and throughput of the center cell for the next day based on the observed network states in the current day. Besides, these performance metrics are not only affected by the current day's states, but also highly correlated with the action we choose to configure for the next day.
Thus, the model is also fed by the actions of the next day. Furthermore, the throughput ratio and throughput of the next day are highly dependent on the previous performance metrics.
Hence, we consider the current throughput ratio, i.e., $\beta_t^v$, in the prediction process. 

To make the final prediction, the learned representation of the neighborhood by the AG-GCN aggregation, the temporal features of the center cell, and the throughput ratio of the current day, i.e. $\beta_t^{v}$, are concatenated to form the state vector of cell $v$ as $\textbf{s}_t^{v} = \big[\beta_t^{v}; \textbf{c}_t^{v}; \textbf{h}_t^{v}\big]$. 
% We define it as: 
% \begin{equation}
%     \textbf{s}_t^{v} = \Big[\beta_t^{v}, \textbf{c}_t^{v}, \textbf{h}_t^{v}\Big].
% \end{equation}
Since the final representation should be sensitive to the chosen input action (of which the decision making process will be elaborated in Sec.~\ref{sec:opt}), the throughput ratio and throughput of the next day for cell $v$ are formulated as the output of a non-linear transformation function of state and action:
\vspace{-0.1cm}
\begin{equation}
    \hat{\beta}_{t+1}^v = \sigma \big( \mathbf{W_{\beta}}.([\textbf{s}_t^{v}; a_t^v])\big),
\end{equation}
\vspace{-0.3cm}
\begin{equation}
    \hat{\alpha}_{t+1}^v = \sigma \big(\mathbf{W_{\alpha}}.([\textbf{s}_t^{v}; a_t^v]) \big).
\end{equation}
\vspace{-0.2cm}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=.5\textwidth]{figures/flowchart.pdf}
% 	\vspace{-.3cm}
% 	\caption{The flow of information from graph structure to final prediction. This flow path is used to form the training pipeline of two models for predicting the throughput $ \hat{\alpha} $ and the throughput ratio $ \hat{\beta} $.}
% 	\label{fig:training_pipeline}
% \end{figure}
The overall flow of data from the graph structure to the final prediction is represented in Fig. \ref{fig:nei_aug_aut_grp}. Note that we train two separate models for predicting the through put and the throughput ratio simultaneously.

The parameter we aim to optimize is the A2-threshold as explain in (\ref{eq:A2_event}).  In order to properly use the A2-threshold for the prediction, we use the change in this parameter compared to the previous day as the action $a_t^v = A2_{t+1}^v - A2_t^v$,
where $A2_{t+1}^v$ and $A2_t^v$ are the A2-thresholds for cell $v$ at day $t+1$ and $t$, respectively.
The reason for this design choice has twofold. First, the original action space of A2 is large, but the range of the change of action can be smaller by controlling the adjustment steps, making it easier for the model to learn and conduct the decision making step. Besides, the delta action directly reflects the change in the cell coverage/loads, so they are more sensitive to the performance metrics.

To form the training objective, we consider data of $T+1$ consecutive days and  form the pairs $(t,t+1)$, $t\in\{1,2,\cdots,T\}$, to predict the throughput ratio and throughput of the center cell in day $T+1$ .
The two models are trained by minimizing the following loss functions respectively:
\vspace{-.2cm}
\begin{equation}
    { {Loss (thrp ratio)}} =  \frac{1}{T}\sum_{t=1}^T\frac{1}{N_t}\sum_{v=1}^{N_t} (\hat{\beta}_{t+1}^v - \beta_{t+1}^v)^2 + \lambda_1||\Theta_1||^2,
\end{equation}
\begin{equation}
     { {Loss (thrp)}}=  \frac{1}{T}\sum_{t=1}^T\frac{1}{N_t}\sum_{v=1}^{N_t} (\hat{\alpha}_{t+1}^v - \alpha_{t+1}^v)^2 + \lambda_2||\Theta_2||^2,
\end{equation}
where $\lambda_1$ and $\lambda_2$ are the hyperparameters chosen for regularization. ${
\Theta}_1$ and ${\Theta}_2$ represent all the trainable parameters in the models. $T$ is the total number of pairs of data used for the training. $N_t$ is the total number of cells available at day $t$. 

The trained reward model is now able to mimic the real network and predict both throughput ratio and throughput of each center cell for the coming day and can be used to check the impact of actions towards the performance metrics we are considering.
The best action is the action that can optimize the throughput ratio and throughput jointly or in other words maximize the optimization problem in (\ref{eq:opt}).



==> sections/appendices.tex <==
\subsection{Baseline comparison}
We summarize the alternative designs for the reward model we consider in our paper in Table \ref{tab:Models}.

\subsection{Simulator Construction}\label{sec:simulator}
The experiments are run by a proprietary cellular network simulator which uses statistical models to simulate the network response to any change in the parameter values. This simulator is designed based on the network corresponding to Dataset-A and uses the states of the network cells along with their action to simulate the throughput and the traffic of the cells.

% \sout{The experiments are conducted on a proprietary cellular network simulator. Here we briefly introduce the methodologies of the simulator construction.}

% \sout{The simulator is constructed from a dataset that is collected from a real metropolitan cellular network containing around 1500 cells. The collection period starts from October 17 to October 31, 2019, where for each day the data of cells are sampled hourly.Each data sample contains information such as the cell ID, sample time, configuration of cell parameters, and measurements of the cell states (e.g., the number of total users within the cell, the number of active users, the cell average CQI, the cell traffic load, etc.) and performance indicators (e.g., the average cell throughput, the edge user throughput, etc.). The neighbor relation information between cells are also collected and the hourly average handover counts between neighbor cells are recorded.}

Dataset-A is collected under the default network configuration and the value of A2-threshold is not changed during the collection period. To evaluate our model and the action configuration strategy, the simulator needs to simulate the network performance given arbitrary A2-threshold values of the cells. More precisely, let $\textbf{x}_t^i$ represents cell $i$'s states at day $t$ under the default A2-threshold configuration, and $A2_t^i$ be the configured A2-threshold value for cell $i$ at day $t$, the simulator will output
\begin{equation}
    \Tilde{\textbf{x}}_t^0, ..., \Tilde{\textbf{x}}_t^{N_t}, r_t^0, ..., r_t^{N_t} = g(\textbf{x}_t^0, ..., \textbf{x}_t^{N_t}, A2_t^0, ...,A2_t^{N_t}),
\end{equation}
where $r^i_{t}$ is cell $i$'s throughput, and $\Tilde{\textbf{x}}_t^{i}$ is the observed states of cell $i$ under the new configurations at $t$.
\begin{figure}[t!]
    \vspace{-.3cm}
    \centering
    \includegraphics[width=.45\textwidth]{figures/simulator_flow.PNG}
    \vspace{-.5cm}
    \caption{The internal workflow of the simulator.}
    \vspace{-.5cm}
    \label{fig:simu_flow}
\end{figure}

Fig.~\ref{fig:simu_flow} gives a simple sketch on the internal workflow of the simulator. During simulation, when $A2_t^0,...,A2_t^{N_t}$ are configured at day $t$, the cell states $\textbf{x}_t^0, ..., \textbf{x}_t^{N_t}$ are read from the collected data, and inputted to the simulator. The cell coverage $C^i$ for each $i$ is first computed by a built-in function that considers cell $i$'s frequency, bandwidth and $A2_t^i$. Then cell $i$'s traffic load (including the number of users and the amount of data bits for transmission) at day $t$ is redistributed among itself and its neighbors based on the change of $C^i$ and $C^j$ with $j \in \mathcal{N}_t(i)$. After each cell's traffic load is updated, the throughput $r_t^i$ is predicted based on cell $i$'s traffic load. The load-throughput prediction model for each cell is pre-trained from the collected historical data and stored when the simulator is initialized. The value $r_t^i$ is further adjusted by a factor that considers the throughput loss due to measurement reporting or connection loss. Finally, the simulator outputs $r_t^0,...,r_t^{N_t}$. As each cell's traffic load (part of the cell states) is modified, the updated states $\Tilde{\textbf{x}}_t^0, ..., \Tilde{\textbf{x}}_t^{N_t}$ are also outputted.

% \subsection{Grouping Schemes Study}\label{sec:grouping_scheme}
% To further investigate the effectiveness of our model, we conduct an ablation study on the auto-grouping module (operator $ \gamma $). To this purpose, the TAG-GCN model is trained using different methods of auto-grouping along with Dataset-B. We use the augmented neighbors set along with different auto-grouping methods as follows:
% 	\begin{itemize}
% 		\item EGNA (Euclidean and Graph Neighbor Augmentation): Our proposed method in this paper.
% 		\item Rule-based: In this method, a simple rule replaces $ \gamma $ where we use two selected features of the neighboring nodes and group the neighbors based on their relative value compared to the corresponding feature of the center node. For instance, if traffic and the value of A2-threshold are chosen (\wm{this is the case in the current study as these features are theoretically the most important ones in the handover process}), all the neighboring nodes of which the traffic and A2-threshold are lower than the center node form the first group, the second group consists of all the neighboring nodes of which the traffic is lower than the center node while the A2-threshold is higher than its counterpart, and so on. {\cj{Maybe need to explain why we chose these two features to compare, since the features we choose may affect the final performance. And another question: since the A2-threshold is the variable we control, does it mean that the neighbor relation will be changed by our action?}}
% 		\item K-Means: Here, the augmented neighbors set is clustered into $ M $ groups, and the groups are sorted based on the distance of the center of each cluster from the center node.
% 		%	\item KMeans2D: This method is similar to KMeans, except that the clustering is performed in the 2D space. The neighbors' features are mapped to a 2D space using PCA after which we use k-means clustering in the previously mentioned fashion. Note that the mapping into 2D space is used to overcome the possible curse of dimensionality in the KMeans method as the number of neighbors can be small compared to the number of features.
% 	\end{itemize}
% % 	The resulting models are trained on Dataset-B in an experiment setup similar to the previous test, e.i., the algorithm is run using 5 different random seeds for the first day recommendation. The MSE curves for testing of the throughput and throughput ratio models are presented in Fig.\ref{fig:AG_Module_MSE}.

% % \begin{figure}
% % 	\subfloat[][]{\includegraphics[width=.245\textwidth]{figures/thrp_test_MSE_TAG-GCN_multi-obj.pdf}}
% % 	\subfloat[][]{\includegraphics[width=.245\textwidth]{figures/ratio_test_MSE_TAG-GCN_multi-obj.pdf}}
% % 	\caption{Mean squared error of the (a) throughput and (b) throughput ratio models for different auto-grouping schemes in TAG-GCN using same dataset.}
% % 	\label{fig:AG_Module_MSE}
% % \end{figure}

% In Fig.~\ref{fig:reward_diff_grouping}, we compare the effect of different grouping schemes on the performance of the network and Table~\ref{tab:reward_diff_grouping} shows the numerical values relative to the best result achieved by the optimal actions.
% As seen, all these grouping achieve very close network performance and our EGNA achieves the best result with a small gap.

% \begin{figure}
% 	% \vspace{-.4cm}
% 	\centering
% 	\includegraphics[width=.475\textwidth]{figures/grouping.pdf}
% 	\vspace{-.8cm}
% 	\caption{Performance comparison of different grouping schemes in TAG-GCN (averaged over 5 trials with random initialization).}
% 	\label{fig:reward_diff_grouping}
% \end{figure}
% % Also Table~\ref{tab:reward_diff_grouping} shows the numerical values corresponding to Fig.\ref{fig:reward_diff_grouping}.
% \begin{table}[]
% 	\centering
% 	\begin{tabular}{|c|c|c|c|} 
% 		\hline
% 		~~ & EGNA & Rule-based & KMeans \\ \hline
% 		\textit{10-28} & 76.12\% & 77.28\% & 77.67\% \\
% 		\textit{10-29} & 84.64\% & 85.54\% & 85.53\% \\
% 		\textit{10-30} & 99.11\% & 100.03\% & 99.35\% \\
% 		\textit{10-31} & 88.08\% & 89.47\% & 89.29\% \\ \hline
% 	\end{tabular}
% % 	\vspace{-.1cm}
% 	\caption{The Average throughput for different grouping schemes divided by the throughput achieved from the best action designed by the simulator (in last four days).}
% 	\label{tab:reward_diff_grouping}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
    \centering
    {\fontsize{7}{8}\selectfont
    \begin{tabular}{|M{1.5cm}||M{.7cm}|M{1.9cm}|M{2.1cm}|}
     \hline
     \multicolumn{4}{|c|}{Model List} \\
     \hline \centering
     Model Name & Graph & Heterogeneous Graph & Daily Temporal Features\\
     \hline
     MLP  & \xmark & \xmark & \xmark\\
     GCN  & \cmark & \xmark & \xmark\\
     AG-GCN  & \cmark & \cmark & \xmark\\
     TAG-GCN  & \cmark & \cmark & \cmark\\
     \hline
    \end{tabular}}
    % \vspace{-.1cm}
    \caption{Properties of Different Models}
    % \vspace{-.6cm}
    \label{tab:Models}
\end{table}

% \subsection{Dataset Samples} \label{sec:dataset_samples}
% We present the values of four different features of three random cells in Dataset-A in Tables~\ref{tab:dataset_A}.
% Note that the represented values are collected in the first day.
% As seen the range of variation across different cells and different hours for each single cell is too high and that is the reason we consider the modules to handle spatial and temporal dependencies in our model to better imitate the real-world environment.
% We have almost the same pattern in Dataset-B as well for these presented features.

% \begin{table}[]
% 	\centering
% 	{\fontsize{7}{8}\selectfont
% 	\begin{tabular}{|M{.4cm}|M{1.1cm}|M{1.4cm}|M{.9cm}|M{1.3cm}|M{.6cm}|} \hline
% 		%L_USER_DL_THROUGPUT_FULLBUFF_MBPS, L_TRAFFIC_USER_AVG, CELL_DLBANDWIDTH, L_AVGCQI
% 		& Time &  Cell Throughput & AVG Traffic & Cell Bandwidth & AVG CQI\\
% 		\hline
% 		& 00 - 01 & 17.18 & 86.14 & 5.0 & 11.84\\
% 		& 01 - 02 & 12.97 & 55.06 & 5.0 & 12.36\\ 
% 		& 02 - 03 & 19.25 & 50.09 & 5.0 & 12.48\\
% 		\vspace{-.5cm} Cell 999 & $\vdots$ & $\vdots$ &$\vdots$ &$\vdots$ &$\vdots$\\
% 		& 23 - 00 & 7.17 & 128.63 & 5.0 & 11.84\\ \cline{2-6}
% 		& Daily AVG & 17.78 & 105.52 & 5.0 & 11.82 \\\hline
		
% % 		& 00 - 01 & 28.48 & 47.17 & 3.0 & 13.69\\
% % 		& 01 - 02 & 36.07 & 36.90 & 3.0 & 13.88\\
% % 		& 02 - 03 & 40.00 & 23.98 & 3.0 & 13.74\\
% % 		\vspace{-.5cm} Cell 1391 & \vdots & \vdots &\vdots &\vdots &\vdots\\
% % 		& 23 - 00 & 18.67 & 52.52 & 3.0 & 13.61\\ \cline{2-6}
% % 		& Daily AVG & 30.29 & 35.37 & 3.00 & 13.86 \\\hline
		
% 		& 00 - 01 & 17.45 & 16.31 & 5.0 & 11.46\\
% 		& 01 - 02 & 24.15 & 11.59 & 5.0 & 10.51\\
% 		& 02 - 03 & 32.26 & 7.36 & 5.0 & 9.49\\
% 		\vspace{-.5cm} Cell 1720 & $\vdots$ & $\vdots$ &$\vdots$ &$\vdots$ &$\vdots$\\
% 		& 23 - 00 & 27.62 & 18.38 & 5.0 & 11.19\\ \cline{2-6}
% 		& Daily AVG & 24.42 & 18.08 & 5.0 & 10.24 \\\hline
		
% 		& 00 - 01 & 26.56 & 15.65 & 5.0 & 11.51\\
% 		& 01 - 02 & 37.82 & 7.52 & 5.0 & 10.97\\ 
% 		& 02 - 03 & 35.80 & 4.62 & 5.0 & 11.53\\
% 		\vspace{-.5cm} Cell 997 & $\vdots$ & $\vdots$ &$\vdots$ &$\vdots$ &$\vdots$\\
% 		& 23 - 00 & 31.41 & 22.94 & 5.0 & 11.67\\ \cline{2-6}
% 		& Daily AVG & 31.05 & 26.72 & 5.0 & 11.48 \\\hline
% 	\end{tabular}
%     }
% 	\caption{Samples from Dataset-A.}
% 	\label{tab:dataset_A}
% \end{table}

% % \begin{table}[]
% % 	\centering
% % 	{\fontsize{7}{8}\selectfont
% % 	\begin{tabular}{|p{.5cm}|p{.8cm}|p{1.6cm}|p{.9cm}|p{1.3cm}|p{.6cm}|} \hline
% % 	\centering
% % 		& Time &  Cell Throughput & AVG Traffic & Cell Bandwidth & AVG CQI\\
% % 		\hline
% % 		& 00 - 01 & 16.83 & 4.35 & 5.0 & 10.10\\
% % 		& 01 - 02 & 22.67 & 7.27 & 5.0 & 9.90\\ 
% % 		& 02 - 03 & 22.94 & 4.99 & 5.0 & 9.75\\
% % 		\vspace{-.5cm} Cell 1284 & \vdots & \vdots &\vdots &\vdots &\vdots\\
% % 		& 23 - 00 & 28.62 & 5.76 & 5.0 & 10.45\\ \cline{2-6}
% % 		& Daily AVG & 17.92 & 7.18 & 5.0 & 10.16 \\\hline
		
% % % 		& 00 - 01 & 23.14 & 5.25 & 3.0 & 11.08\\
% % % 		& 01 - 02 & 35.96 & 4.69 & 3.0 & 10.71\\ 
% % % 		& 02 - 03 & 34.48 & 6.08 & 3.0 & 11.21\\
% % % 		\vspace{-.5cm} Cell 684 & \vdots & \vdots &\vdots &\vdots &\vdots\\
% % % 		& 23 - 00 & 11.57 & 7.39 & 3.0 & 10.10\\ \cline{2-6}
% % % 		& Daily AVG & 15.41 & 6.02 & 3.00 & 9.76 \\\hline
		
% % 		& 00 - 01 & 8.12 & 6.28 & 3.0 & 8.95\\
% % 		& 01 - 02 & 18.22 & 5.73 & 3.0 & 9.12\\ 
% % 		& 02 - 03 & 18.66 & 6.00 & 3.0 & 9.24\\
% % 		\vspace{-.5cm} Cell 1127 & \vdots & \vdots &\vdots &\vdots &\vdots\\
% % 		& 23 - 00 & 14.91 & 7.61 & 3.0 & 8.96\\ \cline{2-6}
% % 		& Daily AVG & 11.09 & 10.38 & 3.0 & 8.98 \\\hline
		
% % 		& 00 - 01 & 32.50 & 29.14 & 5.0 & 10.35\\
% % 		& 01 - 02 & 30.39 & 22.81 & 5.0 & 10.58\\ 
% % 		& 02 - 03 & 33.88 & 22.67 & 5.0 & 10.99\\
% % 		\vspace{-.5cm} Cell 986 & \vdots & \vdots &\vdots &\vdots &\vdots\\
% % 		& 23 - 00 & 29.25 & 37.42 & 5.0 & 10.21\\ \cline{2-6}
% % 		& Daily AVG & 22.45 & 43.41 & 5.0 & 10.32 \\\hline
% % 	\end{tabular}
% %     }
% % 	\caption{Samples from Dataset-B.}
% % 	\label{tab:dataset_B}
% % \end{table}

\begin{figure}
    \vspace{-.5cm}
    \subfloat[][]{\includegraphics[width=.245\textwidth]{figures/TestMSE_old_data_ratio.pdf}}
	\subfloat[][]{\includegraphics[width=.24\textwidth]{figures/TestMSE_new_data_ratio.pdf}}
    % \includegraphics[width=.475\textwidth]{figures/TestMSE_old_data.pdf}
	\vspace{-.45cm}
	\caption{Mean squared error of the throughput ratio for test data of (a) Dataset-A and (b) Dataset-B for TAG-GCN.}
	\vspace{-.4cm}
	\label{fig:TAG-GCN_test_mse_ratio}
\end{figure}




\subsection{Additional Experimental Results}

\subsubsection{Reward Modeling Performance for Throughput Ratio}\label{sec:appendix_mse}
We repeat the same experiment as Fig.~\ref{fig:TAG-GCN_test_mse_thrp} but for the throughput ratio reward and compare the performance measured in the achieved MSE by different models for Dataset-A and B in Fig.~\ref{fig:TAG-GCN_test_mse_ratio}.

\subsubsection{Ablation Study on the Multi-Objective Action Recommendation Strategy} \label{sec:appendix_multi_obj}

In Fig.~\ref{fig:Multi_objPerformance}, we show an ablation study on the effectiveness of our proposed multi-objective action recommendation strategy. 
For each setting, we repeat our experiment five times with TAG-GCN as the reward model but follow different action configuration strategies. Other than the multi-object formulation, we consider two alternatives for action configuration, one by considering only the cell throughput in the optimization problem, and one by considering only the load-balancing objective.
As shown in Fig.~\ref{fig:Multi_objPerformance}, our proposed TAG-GCN model with both load-balancing and throughput as optimization objectives can outperform others, achieving the best average throughput in the final days across random trials.

\subsubsection{The Quantitative Results} \label{sec:appendix_quantitive}

The quantitative results for Fig.~\ref{fig:ModelPerformance} and Fig.~\ref{fig:Multi_objPerformance} are summarized in Table~\ref{tab:num_res_diff_models} and Table~\ref{tab:num_res_diff_opt}, respectively. 
We present the achieved network throughput by different models divided by the performance achieved by the best actions of the simulator for the last 4 days of the experiments. 
As seen, in the first table, the proposed method is outperforming the rest of the methods and yields better average throughput. Furthermore, our method also yields lower variance with respect to change in the initial values of the actions, which is a significant advantage. In general, our method proves to be very robust in this regard.
The second table demonstrates the effectiveness of the multi-objective optimization strategy. 
In this table, we have denoted three different variants of TAG-GCN which represent three optimization strategies, namely, multi-objective strategy using both throughput and throughput ratio models (TAG-GCN1), single objective strategies using throughput ratio (TAG-GCN2), and throughput models (TAG-GCN3). As the results in the table show, the multi-objective strategy outperforms the single objective ones and therefore is superior.

% The quantitative results for Fig.~\ref{fig:Multi_objPerformance} is summarized in Appendix tables~ \ref{tab:num_res_diff_opt}. We present the achieved network throughput by different models divided by the performance achieved by the best actions of the simulator for the last 4 days of the experiments. 
% As seen, in the first table the proposed method is outperforming the rest of the methods and yields better average throughput. {Furthermore, our method also yields lower variance with respect to change in the initial values of the actions, which is a significant advantage. In general, our method proves to be very robust in this regard.} 
% The second table demonstrates the effectiveness of the multi-objective optimization strategy. 
% In this table, we have denoted three different variants of TAG-GCN which represent three optimization strategies, namely, multi-objective strategy using both throughput and throughput ratio models (TAG-GCN1), single objective strategies using throughput ratio (TAG-GCN2), and throughput models (TAG-GCN3). As the res:appults in the table show, the multi-objective strategy outperforms the single objective ones and therefore is superior.

\begin{table}[t]
% 	\vspace{0.5cm}
	\centering
\resizebox{\columnwidth}{!}{%
	\begin{tabular}{|c|c|c|c|c|c|} 
		\hline
		Date & Experts Actions & MLP & GCN & AG-GCN & TAG-GCN\\ \hline
		\textit{10-28} & $0.20 \pm 0.02$ & $0.33 \pm 0.12$ & $0.36 \pm 0.14$ & $0.39 \pm 0.11$ & $\mathbf{0.63 \pm 0.05}$\\
		\textit{10-29} & $0.26 \pm 0.02$ & $0.41 \pm 0.14$ & $0.48 \pm 0.17$ & $0.51 \pm 0.14$ & $\mathbf{0.76 \pm 0.06}$\\
		\textit{10-30} & $0.40 \pm 0.03$ & $0.50 \pm 0.16$ & $0.57 \pm 0.19$ & $0.60 \pm 0.16$ & $\mathbf{0.90 \pm 0.04}$\\
		\textit{10-31} & $0.38 \pm 0.01$ & $0.44 \pm 0.14$ & $0.51 \pm 0.17$ & $0.54 \pm 0.13$ & $\mathbf{0.79 \pm 0.05}$\\ \hline
	\end{tabular}}
% 	\vspace{-.1cm}
	\caption{The Average throughput divided by the throughput achieved from the best action designed by the simulator (in last four days) for different reward models.}
	\vspace{-0.4cm}
	\label{tab:num_res_diff_models}
\end{table}
\vspace{-0.2cm}

\begin{table}[t]
    % \vspace{-0.6cm}
	\centering
	{\fontsize{8}{10}\selectfont
	\begin{tabular}{|c|c|c|c|} 
		\hline
		Date & TAG-GCN1 &  TAG-GCN2 & TAG-GCN3 \\ \hline
		\textit{10-28} & $\mathbf{0.63 \pm 0.05}$ & $0.58 \pm 0.01$ & $0.51 \pm 0.02$ \\
		\textit{10-29} & $\mathbf{0.76 \pm 0.06}$ & $0.66 \pm 0.01$ & $0.60 \pm 0.03$ \\
		\textit{10-30} & $\mathbf{0.90 \pm 0.04}$ & $0.73 \pm 0.01$ & $0.65 \pm 0.06$ \\
		\textit{10-31} & $\mathbf{0.79 \pm 0.05}$ & $0.71 \pm 0.02$ & $0.65 \pm 0.03$ \\ \hline
	\end{tabular}}
% 	\vspace{-.1cm}
	\caption{The 95\% confidence interval for the average throughput divided by the throughput achieved from the best action designed by the simulator (in last four days) for different optimization methods using TAG-GCN model.}
	\label{tab:num_res_diff_opt}
\end{table}


\begin{figure}[t!]
    \vspace{-.5cm}
    \centering
    \includegraphics[width=.475\textwidth]{figures/opt.pdf}
    \vspace{-.8cm}
    \caption{The impact of different optimization objectives for the parameter configuration in our proposed TAG-GCN model.}
    \vspace{-.3cm}
    \label{fig:Multi_objPerformance}
\end{figure}

\subsubsection{Different action initialization strategies}\label{sec:appendix_init}
In Fig.~\ref{fig:InitializationPerformance}, we present an ablation study on the different initialization schemes on the first action exploration day.
In addition to the random initialization, we use two more action initialization schemes including the expert rule and the negative slope.
The expert rule initialization is given in (\ref{eq:experts}), where at day $t+1$, the actions are set for each cell $v\in N_t$ based on the load balancing as:
% \vspace{-0.2cm}
\begin{equation}\label{eq:experts}
    a_t^v = \begin{cases}
r_1^v(\beta_{t}^v-1) &\beta_{t}^v\ge 1\\
r_2^v(\beta_{t}^v-1) &\beta_{t}^v<1
\end{cases},
\end{equation}
where $r_1^v, r_2^v < 0$ are the weights set by human experts. The intuition is to increase the A2-threshold to release traffic when a cell is overloaded and decrease the value in the opposite case.
The negative slope procedure for the action initialization is defined based on the throughput ratio of the first day of each cell $v$, i.e., $\beta_{t_1}^{v}$ as $a_{t_1}^{v} = \Big[\frac{2(\beta_{t_1}^{v} - \rho)\phi}{\rho - \tau} + \phi\Big]$,
% \begin{equation}
%     a_{t_1}^{v} = -100 + \Big[\frac{2(\beta_{t_1}^{v} - \rho)\phi}{\rho - \tau} + \phi\Big],
% \end{equation}
where $\rho = \min_{v\in N_{t_1}}(\beta_{t_1}^{v})$, and $\tau = \max_{v\in N_{t_1}}(\beta_{t_1}^{v})$ and $[\cdot]$ is the rounding operation.
% $N_{t_1}$ is the number of cells in the dataset at day $t_1$. 
For controlling the variation of action, the maximum range of change is defined as $\phi$. We can observe that regardless of the type of initialization, the model can converge to almost the same performance in the final days, which indicates that even without strong prior information from the network, our design can still quickly converge to the desired model performance.


\begin{figure}[t!]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=.475\textwidth]{figures/init.pdf}
    \vspace{-.8cm}
    \caption{Performance comparison of the TAG-GCN model under different types of action initialization for Oct. 18.}
    \vspace{-.4cm}
    \label{fig:InitializationPerformance}
\end{figure}
%with a specified reward function
\subsection{Reinforcement Learning Modeling} \label{sec:appendix_rl}
As we mentioned in section~\ref{sec:benchmark}, for problems similar to ours which require following a policy to choose an action to interact with an environment, reinforcement learning (RL) modeling is a good candidate. 
Among all the RL methods, actor-critic (AC) method is a potential match to our problem due to its continuous action space and modeling flexibility.
AC methods have been widely used in cellular network problems and for different tasks such as power allocation and traffic forecasting \cite{AC_traffic, AC_thrp, AC_iot, AC_resal}.  
Hence, as an additional benchmark we compare our proposed algorithm with a basic AC algorithm we implemented to adapt to our problem where the actor model recommends actions in order to maximize the reward predicted by the critic model.

We use TAG-GCN as the critic model to predict the reward which can be either throughput ratio or throughput to train the actor model. 
For the actor model, we use the same modules presented for TAG-GCN to do the neighbor auto-grouping and capture the temporal dependencies in the data and train it with the following loss function
\begin{equation}
    { {Loss (actor)}}=  \frac{1}{T}\sum_{t=1}^T\frac{1}{N_t}\sum_{v=1}^{N_t} \sqrt{\big|1-\hat{\beta}_t^{v}(\hat{a}_t^v)\big|} + \lambda_3||\Theta_3||^2,
\end{equation}
where $\hat{a}_t^v$ is the recommended action by the actor model and $\hat{\beta}_t^{v}(\hat{a}_t^v)$ is the predicted reward by the critic model using the recommended action.  
$\lambda_3$ is the hyperparameter chosen for regularization and ${\Theta}_3$ represents all the trainable parameters in the actor model.

Fig.~\ref{fig:AC} shows that TAG-GCN outperforms this basic RL model. The proposed AC model is a very preliminary one and obviously it can be improved even more which is out of the scope of this paper. 
However, this potential improvement comes with the cost of increasing complexity and requires a highly diverse data and more interactions with the environment.
The RL approach generally requires frequent and plenty of interactions with the environment. However, in our case, the action is configured once a day, and the total exploration duration only consists of 11 days, which is far less than what is generally required by the RL models.
Furthermore, RL models usually consider accumulated returns, i.e., impact of the current action on the future performance. However, in our scenario, the current action only affects the loads distribution of the current hour, and does not affect the future performance. Therefore the standard RL approach does not apply here.

% \begin{enumerate}
%     \item The RL approach generally requires frequent and plenty of interactions with the environment. However, in our case, the action is configured once a day, and the total exploration duration only consists of 11 days, which is far less than what is generally required by the RL models. 
%     \item RL models usually considers accumulated returns, i.e., impact on the future performance of the current action. However, in our scenario, the current action only affects the loads distribution of the current hour, and does not affect the future performance. Therefore the standard RL approach does not apply here.
% \end{enumerate}

% the comparison between our proposed model and the AC model we introduced. 
% As seen our model can beat the AC model by using two objectives and this improvement achieved with less complexity.
% In Table~\ref{tab:AC}, we compare the computational time of different methods using either our action exploration or using AC strategy to find the best action.

% {\cj{I think this might not be an appropriate comparison. \textit{Reinforcement learning} is a very broad term and consists of many different models. There are even many different variations for \textit{actor critic}. So it is very hard to justify we are using the best RL model for comparison. For example, some RL algorithm also considers multi-objective problems, which seems to be more suitable in this case. 

% In addition, the actor critic model described here is not a standard implementation of AC (standard AC considers accumulated returns and has a much more complicated form than ours), so the reviewers might be confused by the model.

% To justify we are not using deep reinforcement learning, I think we may state the following reasons:


% 1) we try RL. doesn't provide many advantages 2) It is not the perfect one we tried, just preliminary ones. 3) RL is not suitable for our setting.


\begin{figure}[t!]
    \centering
    \includegraphics[width=.475\textwidth]{figures/AC.pdf}
    \vspace{-.8cm}
    \caption{Performance comparison between our proposed design and actor-critic design for action exploration.}
    \vspace{-.2cm}
    \label{fig:AC}
\end{figure}

% \begin{table}[]
% 	\centering
% 	\begin{tabular}{|c|c|c|c|c|} \hline
% 		&  MLP & GCN & AG-GCN & TAG-GCN \\ \hline
% 		Actor/Critic & 1883.36 & 1941.33 & 2927.75 & 3276.33 \\
% 		Our Method & 1808.66 & 1859.76 & 2895.53 & 3140.88 \\ \hline
% 	\end{tabular}
% 	\caption{Computation time (sec) of different methods}
% 	\label{tab:AC}
% \end{table}
